Orientation reversal of manifolds

We call a closed, connected, orientable manifold in one of the categories TOP, PL or DIFF chiral if it does not admit an orientation-reversing automorphism and amphicheiral otherwise. Moreover, we call a manifold strongly chiral if it does not admit a self-map of degree -1. We prove that there are strongly chiral, smooth manifolds in every oriented bordism class in every dimension greater than two. We also produce simply-connected, strongly chiral manifolds in every dimension greater than six. For every positive integer k, we exhibit lens spaces with an orientation-reversing self-diffeomorphism of order 2^k but no self-map of degree -1 of smaller order.

==> xypdf-co.tex <==
%auto-ignore
%%
%% This is file `xypdf-co.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `color')
%%
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://www.math.uni-bonn.de/people/muellner>
%% --------------------------------------------------------------------------
%%
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%%
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%%
%% --------------------------------------------------------------------------
%%
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%%
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%%
%% The files with the TeX code are generated by the following command:
%%
%%    latex xypdf.ins
%%
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%%
%% --------------------------------------------------------------------------
%%
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%%
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%%

\xycatcodes
\expandafter\let\csname xypdf-co@loaded\endcsname\@empty
\@ifdefinable\xP@colorname\relax
\@ifdefinable\xP@colA\relax
\@ifdefinable\xP@colB\relax
\@ifdefinable\xP@colC\relax
\@ifdefinable\xP@colD\relax
\xP@hook{color}{newxycolor}
\newcommand*\xP@newxycolor[2]{\def\xP@colorname{#1}\xP@parsecolor#2 @}
\@ifdefinable\xP@parsecolor\relax
\def\xP@parsecolor#1 #2 #3@{\def\xP@colA{#1}\def\xP@colB{#2}\ifx\xP@colB\xP@gray
\xP@newcolor\xP@colorname\xP@colA\xP@gray\newxycolor
\else
\xP@parsecolor@#3 @\fi
}
\@ifdefinable\xP@parsecolor@\relax
\def\xP@parsecolor@#1 #2 #3 #4@{\def\xP@colC{#1}\def\xP@colD{#2}\ifx\xP@colD\xP@rgb
\xP@newcolor\xP@colorname{\xP@colA,\xP@colB,\xP@colC}\xP@rgb\newxycolor
\else
\def\@tempa{#3}\ifx\@tempa\xP@cmyk
\xP@newcolor\xP@colorname{\xP@colA,\xP@colB,\xP@colC,\xP@colD}{cmyk}\newxycolor
\else
\PackageError{xypdf}{Syntax error in \string\newxycolor}{}\fi
\fi
}
\newcommand*\xP@gray{gray}
\newcommand*\xP@rgb{rgb}
\newcommand*\xP@cmyk{cmyk}
\xP@hook{color}{OBJECT@shape}
\newcommand*\xP@OBJECT@shape[1]{\DN@{shape [#1]}\expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
\ifx\nextii@\relax\DN@{style [#1]}\expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
\ifx\nextii@\relax\DN@{\xP@checkcolor{#1}}\else\DN@{\nextii@\xyFN@\OBJECT@}\fi
\else\expandafter\addtotoks@\expandafter{\nextii@}\DN@{\xyFN@\OBJECT@}\fi \next@}
\newcommand*\xP@checkcolor[1]{\@ifundefined{\string\color@\detokenize{#1}}{\OBJECT@shapei[#1]}{\xP@append\toks@{\noexpand\xP@color{{\detokenize{#1}}}}\xyFN@\OBJECT@
}}
\newcommand*\xP@color[1]{\def\preStyle@@{\addtostyletoks@{\bgroup\xP@protectedcolor#1}}\def\postStyle@@{\addtostyletoks@{\egroup}}\modXYstyle@
}
\@ifdefinable\xP@protectedcolor\relax
\protected\def\xP@protectedcolor{\@ifundefined{color}\xP@pdfcolor\color
}
\@ifdefinable\xP@pdfcolor\relax
\def\xP@pdfcolor[#1]#2{\edef\@tempa{#1}\ifx\@tempa\xP@gray
\DN@{\xP@graycolor{#2}}\else\ifx\@tempa\xP@rgb
\DN@{\xP@rgbcolor#2@}\else\ifx\@tempa\xP@cmyk
\DN@{\xP@cmykcolor#2@}\fi\fi\fi
\aftergroup\xP@resetcolor
\next@
}\newcommand*\xP@graycolor[1]{\xP@setcolor{#1}gG}\@ifdefinable\xP@rgbcolor\relax
\def\xP@rgbcolor#1,#2,#3@{\xP@setcolor{#1 #2 #3}{rg}{RG}}
\@ifdefinable\xP@cmykcolor\relax
\def\xP@cmykcolor#1,#2,#3,#4@{\xP@setcolor{#1 #2 #3 #4}kK}
\newcommand*\xP@newcolor[4]{\expandafter\let\expandafter\next@\csname shape [#1]\endcsname
\ifx\next@\relax
\@ifundefined{\string\color@#1}\relax
{\xP@warning{xypdf}{The color `#1' is overridden by \string#4}}\DN@{\newxystyle{#1}{\xP@unnamedcolor{#2}{#3}}}\else
\DN@{}\fi
\next@\relax}
\newcommand*\xP@unnamedcolor[2]{\xP@color{[#2]{#1}}}
\newcommand\xP@definecrayolacolor[2]{\xP@newcolor{#1}{#2}{cmyk}\UseCrayolaColors}\newcommand*\xP@installCrayolaColors{\xP@definecrayolacolor{GreenYellow}{.15,0,.69,0}\xP@definecrayolacolor{Yellow}{0,0,1,0}\xP@definecrayolacolor{Goldenrod}{0,.1,.84,0}\xP@definecrayolacolor{Dandelion}{0,.29,.84,0}\xP@definecrayolacolor{Apricot}{0,.32,.52,0}\xP@definecrayolacolor{Peach}{0,.5,.7,0}\xP@definecrayolacolor{Melon}{0,.46,.5,0}\xP@definecrayolacolor{YellowOrange}{0,.42,1,0}\xP@definecrayolacolor{Orange}{0,.61,.87,0}\xP@definecrayolacolor{BurntOrange}{0,.51,1,0}\xP@definecrayolacolor{Bittersweet}{0,.75,1,.24}\xP@definecrayolacolor{RedOrange}{0,.77,.87,0}\xP@definecrayolacolor{Mahogany}{0,.85,.87,.35}\xP@definecrayolacolor{Maroon}{0,.87,.68,.32}\xP@definecrayolacolor{BrickRed}{0,.89,.94,.28}\xP@definecrayolacolor{Red}{0,1,1,0}\xP@definecrayolacolor{OrangeRed}{0,1,.5,0}\xP@definecrayolacolor{RubineRed}{0,1,.13,0}\xP@definecrayolacolor{WildStrawberry}{0,.96,.39,0}\xP@definecrayolacolor{Salmon}{0,.53,.38,0}\xP@definecrayolacolor{CarnationPink}{0,.63,0,0}\xP@definecrayolacolor{Magenta}{0,1,0,0}\xP@definecrayolacolor{VioletRed}{0,.81,0,0}\xP@definecrayolacolor{Rhodamine}{0,.82,0,0}\xP@definecrayolacolor{Mulberry}{.34,.9,0,.02}\xP@definecrayolacolor{RedViolet}{.07,.9,0,.34}\xP@definecrayolacolor{Fuchsia}{.47,.91,0,.08}\xP@definecrayolacolor{Lavender}{0,.48,0,0}\xP@definecrayolacolor{Thistle}{.12,.59,0,0}\xP@definecrayolacolor{Orchid}{.32,.64,0,0}\xP@definecrayolacolor{DarkOrchid}{.4,.8,.2,0}\xP@definecrayolacolor{Purple}{.45,.86,0,0}\xP@definecrayolacolor{Plum}{.5,1,0,0}\xP@definecrayolacolor{Violet}{.79,.88,0,0}\xP@definecrayolacolor{RoyalPurple}{.75,.9,0,0}\xP@definecrayolacolor{BlueViolet}{.86,.91,0,.04}\xP@definecrayolacolor{Periwinkle}{.57,.55,0,0}\xP@definecrayolacolor{CadetBlue}{.62,.57,.23,0}\xP@definecrayolacolor{CornflowerBlue}{.65,.13,0,0}\xP@definecrayolacolor{MidnightBlue}{.98,.13,0,.43}\xP@definecrayolacolor{NavyBlue}{.94,.54,0,0}\xP@definecrayolacolor{RoyalBlue}{1,.5,0,0}\xP@definecrayolacolor{Blue}{1,1,0,0}\xP@definecrayolacolor{Cerulean}{.94,.11,0,0}\xP@definecrayolacolor{Cyan}{1,0,0,0}\xP@definecrayolacolor{ProcessBlue}{.96,0,0,0}\xP@definecrayolacolor{SkyBlue}{.62,0,.12,0}\xP@definecrayolacolor{Turquoise}{.85,0,.2,0}\xP@definecrayolacolor{TealBlue}{.86,0,.34,.02}\xP@definecrayolacolor{Aquamarine}{.82,0,.3,0}\xP@definecrayolacolor{BlueGreen}{.85,0,.33,0}\xP@definecrayolacolor{Emerald}{1,0,.5,0}\xP@definecrayolacolor{JungleGreen}{.99,0,.52,0}\xP@definecrayolacolor{SeaGreen}{.69,0,.5,0}\xP@definecrayolacolor{Green}{1,0,1,0}\xP@definecrayolacolor{ForestGreen}{.91,0,.88,.12}\xP@definecrayolacolor{PineGreen}{.92,0,.59,.25}\xP@definecrayolacolor{LimeGreen}{.5,0,1,0}\xP@definecrayolacolor{YellowGreen}{.44,0,.74,0}\xP@definecrayolacolor{SpringGreen}{.26,0,.76,0}\xP@definecrayolacolor{OliveGreen}{.64,0,.95,.4}\xP@definecrayolacolor{RawSienna}{0,.72,1,.45}\xP@definecrayolacolor{Sepia}{0,.83,1,.7}\xP@definecrayolacolor{Brown}{0,.81,1,.6}\xP@definecrayolacolor{Tan}{.14,.42,.56,0}\xP@definecrayolacolor{Gray}{0,0,0,.5}\xP@definecrayolacolor{Black}{0,0,0,1}\xP@definecrayolacolor{White}{0,0,0,0}}
\xywithoption{crayon}{\xP@installCrayolaColors
\renewcommand*\installCrayolaColors@{}}
\xyendinput
%%
%% End of file `xypdf-co.tex'.


==> xypdf-cu.tex <==
%auto-ignore
%%
%% This is file `xypdf-cu.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `curve')
%%
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://www.math.uni-bonn.de/people/muellner>
%% --------------------------------------------------------------------------
%%
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%%
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%%
%% --------------------------------------------------------------------------
%%
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%%
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%%
%% The files with the TeX code are generated by the following command:
%%
%%    latex xypdf.ins
%%
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%%
%% --------------------------------------------------------------------------
%%
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%%
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%%

\xycatcodes
\expandafter\let\csname xypdf-cu@loaded\endcsname\@empty
\newcommand*\xP@tempvar[2]{\@ifdefinable#1\relax
\let#1#2}
\xP@tempvar\xP@bigdim\quotPTK@
\xP@tempvar\xP@parA\L@p
\xP@tempvar\xP@velA\U@p
\xP@tempvar\xP@parB\R@p
\xP@tempvar\xP@velB\D@p
\xP@tempvar\xP@parC\X@origin
\xP@tempvar\xP@velC\Y@origin
\xP@tempvar\xP@parD\X@xbase
\xP@tempvar\xP@velD\Y@xbase
\xP@tempvar\xP@parE\X@ybase
\xP@tempvar\xP@velE\Y@ybase
\xP@tempvar\xP@lenA\X@min
\xP@tempvar\xP@lenB\Y@min
\xP@tempvar\xP@partlen\X@max
\xP@tempvar\xP@oldpartlen\Y@max
\xP@tempvar\xP@tolerance\almostz@
\xP@tempvar\xP@A\L@p
\xP@tempvar\xP@B\U@p
\xP@tempvar\xP@C\R@p
\xP@tempvar\xP@D\D@p
\xP@tempvar\xP@E\X@origin
\xP@tempvar\xP@F\Y@origin
\xP@tempvar\xP@G\X@xbase
\xP@tempvar\xP@H\Y@xbase
\xP@tempvar\xP@I\X@ybase
\xP@tempvar\xP@J\Y@ybase
\xP@tempvar\xP@K\X@min
\xP@tempvar\xP@L\Y@min
\xP@tempvar\xP@fa\X@max
\xP@tempvar\xP@fd\Y@max
\xP@tempvar\xP@tm\almostz@
\xP@tempvar\xP@xm\K@dXdY
\xP@tempvar\xP@ym\K@dYdX
\@tempcnta\count11\relax
\xP@newdimen\xP@off
\xP@newdimen\xP@ta
\xP@newdimen\xP@tb
\xP@newdimen\xP@tc
\xP@newdimen\xP@M
\xP@newdimen\xP@oldobj
\xP@newdimen\xP@Tax
\xP@newdimen\xP@Tay
\xP@newdimen\xP@Tdx
\xP@newdimen\xP@Tdy
\xP@newdimen\xP@Tmx
\xP@newdimen\xP@Tmy
\xP@newdimen\xP@xa
\xP@newdimen\xP@ya
\xP@newdimen\xP@xb
\xP@newdimen\xP@yb
\xP@newdimen\xP@xc
\xP@newdimen\xP@yc
\xP@newdimen\xP@xd
\xP@newdimen\xP@yd
\count11\@tempcnta
\xP@tempvar\xP@a\X@ybase
\xP@tempvar\xP@b\Y@ybase
\xP@tempvar\xP@c\X@min
\xP@tempvar\xP@valA\Y@min
\xP@tempvar\xP@valB\X@max
\xP@tempvar\xP@devA\Y@max
\xP@tempvar\xP@devB\almostz@
\xP@tempvar\xP@ti\K@dXdY
\xP@tempvar\xP@tip\K@dYdX
\xP@tempvar\xP@sa\xP@Tax
\xP@tempvar\xP@sb\xP@Tay
\xP@tempvar\xP@sc\xP@Tdx
\xP@tempvar\xP@Ab\xP@Tdy
\xP@tempvar\xP@AAb\xP@Tmx
\xP@tempvar\xP@Aba\xP@Tmy
\xP@tempvar\xP@Abb\xP@xa
\xP@tempvar\xP@Abc\xP@ya
\xP@tempvar\xP@AAba\xP@xb
\xP@tempvar\xP@AAbb\xP@yb
\xP@tempvar\xP@AAbc\xP@xc
\xP@tempvar\xP@dta\xP@yc
\xP@tempvar\xP@dtb\xP@xd
\xP@tempvar\xP@dtc\xP@yd
\xP@tempvar\xP@temppar\X@origin
\xP@tempvar\xP@tempvel\Y@origin
\xP@tempvar\xP@posX\X@xbase
\xP@tempvar\xP@posY\Y@xbase
\xP@tempvar\xP@oldpar\X@ybase
\xP@tempvar\xP@lastpar\Y@ybase
\xP@tempvar\xP@tempvel@\X@min
\xP@tempvar\xP@parinc\Y@min
\xP@tempvar\xP@squiglen\almostz@
\xP@tempvar\xP@scaleone\K@
\xP@tempvar\xP@scaletwo\KK@
\xP@tempvar\xP@scalethree\Direction
\xP@hook{curve}{splinesolid@}
\newcommand*\xP@splinesolid@{\xP@spline\xP@setsolidpat}
\xP@hook{curve}{splinedashed@}
\newcommand*\xP@splinedashed@{\xP@spline\xP@setdashpat}
\xP@hook{curve}{splinedotted@}
\newcommand*\xP@splinedotted@{\xP@spline\xP@setdottedpat}
\newcommand*\xP@spline[1]{\readsplineparams@
\ifdim\dimen5<\dimen7
\xP@preparespline
\ifdim\@tempdimb>\z@
#1\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\L@c\U@c\xP@coor\R@c\D@c\xP@coor\X@c\Y@c c}\xP@savec
\fi
\fi
}
\newcommand*\xP@preparespline{\ifx\splineinfo@\squineinfo@
\L@c\dimexpr(\X@p+2\A@)/3\relax
\U@c\dimexpr(\Y@p+2\B@)/3\relax
\R@c\dimexpr(\X@c+2\A@)/3\relax
\D@c\dimexpr(\Y@c+2\B@)/3\relax
\fi
\xP@shavespline
\xP@bezierlength
}
\newcommand*\xP@inibigdim{\xP@bigdim5040pt}
\newcommand*\xP@shavespline{\xP@shaveprec{\dimen5*\xP@bigdim/\p@}{\dimen7*\xP@bigdim/\p@}}
\newcommand*\xP@shaveprec[2]{{\xP@inibigdim
\A@\dimexpr#1\relax
\B@\dimexpr#2\relax
\@tempswatrue
\ifdim\A@=\z@\ifdim\B@=\xP@bigdim\@tempswafalse\fi\fi
\if@tempswa
\L@p\dimexpr\L@c-\X@p\relax
\U@p\dimexpr\R@c-\L@p-\L@c\relax
\R@p\dimexpr\X@c-3\R@c+3\L@c-\X@p\relax
\D@p\dimexpr\U@c-\Y@p\relax
\X@min\dimexpr\D@c-\D@p-\U@c\relax
\Y@min\dimexpr\Y@c-3\D@c+3\U@c-\Y@p\relax
\xdef\@gtempa{\X@p\the\dimexpr\X@p+(3\L@p+(3\U@p+\R@p*\A@/\xP@bigdim)*\A@/\xP@bigdim)*\A@/\xP@bigdim\relax
\Y@p\the\dimexpr\Y@p+(3\D@p+(3\X@min+\Y@min*\A@/\xP@bigdim)*\A@/\xP@bigdim)*\A@/\xP@bigdim\relax
\L@c\the\dimexpr\X@p+(2\A@+\B@)*\L@p/\xP@bigdim+((\A@+2\B@)*\U@p/\xP@bigdim+\R@p*\A@/\xP@bigdim*\B@/\xP@bigdim)*\A@/\xP@bigdim\relax
\U@c\the\dimexpr\Y@p+(2\A@+\B@)*\D@p/\xP@bigdim+((\A@+2\B@)*\X@min/\xP@bigdim+\Y@min*\A@/\xP@bigdim*\B@/\xP@bigdim)*\A@/\xP@bigdim\relax
\R@c\the\dimexpr\X@p+(2\B@+\A@)*\L@p/\xP@bigdim+((\B@+2\A@)*\U@p/\xP@bigdim+\R@p*\B@/\xP@bigdim*\A@/\xP@bigdim)*\B@/\xP@bigdim\relax
\D@c\the\dimexpr\Y@p+(2\B@+\A@)*\D@p/\xP@bigdim+((\B@+2\A@)*\X@min/\xP@bigdim+\Y@min*\B@/\xP@bigdim*\A@/\xP@bigdim)*\B@/\xP@bigdim\relax
\X@c\the\dimexpr\X@p+(3\L@p+(3\U@p+\R@p*\B@/\xP@bigdim)*\B@/\xP@bigdim)*\B@/\xP@bigdim\relax
\Y@c\the\dimexpr\Y@p+(3\D@p+(3\X@min+\Y@min*\B@/\xP@bigdim)*\B@/\xP@bigdim)*\B@/\xP@bigdim\relax}\else
\global\let\@gtempa\relax
\fi
}\@gtempa
}
\newcommand*\xP@bezierlength{{\xP@inibigdim
\@tempdimb\z@
\xP@parA\z@
\xP@velocity\z@\xP@velA
\xP@parC.5\xP@bigdim
\xP@velocity\xP@parC\xP@velC
\xP@velocity\xP@bigdim\xP@velE
\xP@oldpartlen\dimexpr(\xP@velA+4\xP@velC+\xP@velE)/6\relax
\xP@tolerance\xP@max{1sp}{\dimexpr\xP@oldpartlen/100000\relax}\xP@arclength\xP@parC\xP@velC\xP@bigdim\xP@velE\xP@oldpartlen
\global\dimen@i\@tempdimb
}\@tempdimb\dimen@i
}
\newcommand*\xP@velocity[2]{{\@tempdima\dimexpr#1\relax
\xP@tangent
\global\dimen@i\@tempdimb
}#2\dimen@i
}
\newcommand*\xP@tangent{\d@X3\xP@precbeziertan\X@p\L@c\R@c\X@c\@tempdima
\d@Y3\xP@precbeziertan\Y@p\U@c\D@c\Y@c\@tempdima
\xP@veclen
}
\newcommand*\xP@tangentvec[1]{{\@tempdima#1\relax
\xP@tangent
\ifdim\@tempdimb=\z@
\L@p\dimexpr\X@c-\X@p+(\L@c-\R@c)*3\relax
\U@p\dimexpr\Y@c-\Y@p+(\U@c-\D@c)*3\relax
\d@X\dimexpr\L@p*\@tempdima/\xP@bigdim+(\X@p-2\L@c+\R@c)\relax
\d@Y\dimexpr\U@p*\@tempdima/\xP@bigdim+(\Y@p-2\U@c+\D@c)\relax
\xP@veclen
\ifdim\@tempdimb=\z@
\d@X\L@p
\d@Y\U@p
\xP@veclen
\ifdim\@tempdimb=\z@
\xP@warning{xypdf}{Cannot determine a tangent vector to a curve}\@tempdimb\p@
\fi
\fi
\fi
\global\dimen@i\d@X
\global\dimen3\d@Y
\global\dimen5\@tempdimb
}\d@X\dimen@i
\d@Y\dimen3\relax
\@tempdimb\dimen5\relax
}
\newcommand*\xP@arclength[5]{\xP@parE#3\xP@velE#4\xP@parC#1\xP@velC#2\xP@oldpartlen#5\xP@parB\dimexpr(\xP@parC+\xP@parA)/2\relax
\xP@velocity\xP@parB\xP@velB
\xP@parD\dimexpr(\xP@parE+\xP@parC)/2\relax
\xP@velocity\xP@parD\xP@velD
\xP@lenA
\dimexpr(\xP@velA+4\xP@velB+\xP@velC)/6*(\xP@parC-\xP@parA)/\xP@bigdim\relax
\xP@lenB
\dimexpr(\xP@velC+4\xP@velD+\xP@velE)/6*(\xP@parE-\xP@parC)/\xP@bigdim\relax
\xP@partlen\dimexpr\xP@lenA+\xP@lenB\relax
{\@tempdima\dimexpr\xP@oldpartlen-\xP@partlen\relax
\expandafter}\ifdim\ifdim\@tempdima<\z@-\fi\@tempdima>\xP@tolerance
\edef\next@{\noexpand\xP@arclength\xP@parB\xP@velB\xP@parC\xP@velC\xP@lenA
\noexpand\xP@arclength{\the\xP@parD}{\the\xP@velD}{\the\xP@parE}{\the\xP@velE}{\the\xP@lenB}}\else
\xP@parA\xP@parE
\xP@velA\xP@velE
\advance\@tempdimb\xP@partlen
\DN@{}\fi
\next@
}
\xP@hook{curve}{@crv@}
\newcommand*\xP@@crv@[2]{\DN@{#1#2}\ifx\next@\@empty \edef\next@{\crv@defaultshape}\ifx\bstartPLACE@\@empty\xdef\crvSTYLE@@{{\crv@defaultshape}}\fi
\else
\ifx\bstartPLACE@\@empty\gdef\crvSTYLE@@{#1{#2}}\fi
\fi
\ifx\next@\@empty\crv@noobject \DN@{\crv@{}{\xy@@crvaddstack@}}\else\def\tmp@{-}\ifx\next@\tmp@ \DN@{\crv@{}{\xy@@crvaddstack@}}\else\def\tmp@{=}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{=}}}\else\def\tmp@{2-}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{2.}}}\else\def\tmp@{3-}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{3.}}}\else\def\tmp@{--}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@specialtemplate@{--}}\else\def\tmp@{==}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}\else\def\tmp@{2--}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}\else\def\tmp@{3--}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{--}}}\else\def\tmp@{.}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@specialtemplate@{.}}\else\def\tmp@{:}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}\else\def\tmp@{2.}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}\else\def\tmp@{3.}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{.}}}\else\def\tmp@{~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{~}}}\else\def\tmp@{2~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{~}}}\else\def\tmp@{3~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{~}}}\else\def\tmp@{~~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{~~}}}\else\def\tmp@{2~~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{~~}}}\else\def\tmp@{3~~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{~~}}}\else\def\tmp@{..}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@specialtemplate@{.}}\else
\DN@{\expandafter\crv@\crv@othertemplate{\dir#1{#2}}}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\next@}
\xP@hook{curve}{xysplinespecialcases@}
\newcommand*\xP@xysplinespecialcases@{\ifx\@empty\xycrvdrop@
\ifx\@empty\xycrvconn@\DN@{\splinesolid@}\else\DN@{ \dir{-}}\ifx\next@\xycrvconn@\DN@{\splinesolid@}\else\DN@{ \dir2{-}}\ifx\next@\xycrvconn@\DN@{\splinedoubled@}\else\DN@{ \dir{=}}\ifx\next@\xycrvconn@\DN@{\splineribboned@}\else\DN@{ \dir{2.}}\ifx\next@\xycrvconn@\DN@{\splinedoubled@}\else\DN@{ \dir3{-}}\ifx\next@\xycrvconn@\DN@{\splinetrebled@}\else\DN@{ \dir{3.}}\ifx\next@\xycrvconn@\DN@{\splinetrebled@}\else\DN@{ \dir{--}}\ifx\next@\xycrvconn@\DN@{\splinedashed@}\else\DN@{ \dir{.}}\ifx\next@\xycrvconn@\DN@{\splinedotted@}\else\DN@{ \dir{:}}\ifx\next@\xycrvconn@\DN@{\splinedbldotted@}\else\DN@{ \dir2{.}}\ifx\next@\xycrvconn@\DN@{\splinedbldotted@}\else\DN@{ \dir3{.}}\ifx\next@\xycrvconn@\DN@{\xP@splinetrbldotted}\else\DN@{ \dir2{--}}\ifx\next@\xycrvconn@\DN@{\xP@splinedbldashed}\else\DN@{ \dir3{--}}\ifx\next@\xycrvconn@\DN@{\xP@splinetrbldashed}\else\DN@{ \dir{~}}\ifx\next@\xycrvconn@\DN@{\xP@splinesquiggled}\else\DN@{ \dir2{~}}\ifx\next@\xycrvconn@\DN@{\xP@splinedblsquiggled}\else\DN@{ \dir3{~}}\ifx\next@\xycrvconn@\DN@{\xP@splinetrblsquiggled}\else\DN@{ \dir{~~}}\ifx\next@\xycrvconn@\DN@{\xP@splinebrokensquiggled}\else\DN@{ \dir2{~~}}\ifx\next@\xycrvconn@\DN@{\xP@splinebrokendblsquiggled}\else\DN@{ \dir3{~~}}\ifx\next@\xycrvconn@\DN@{\xP@splinebrokentrblsquiggled}\else\ifdim\splinetol@>\z@\else\splinedefaulttol@\fi
\DN@{\splineset@@}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\else
\DN@{\splineset@@}\fi
\ifInvisible@\DN@{}\fi
\next@
}
\xP@hook{curve}{splinedoubled@}
\newcommand*\xP@splinedoubled@{\xP@checkspline\xP@splinemultsolid\xP@doublestroke}
\xP@hook{curve}{splineribboned@}
\@ifdefinable\xP@splineribboned@\relax
\let\xP@splineribboned@\xP@splinedoubled@
\xP@hook{curve}{splinetrebled@}
\newcommand*\xP@splinetrebled@{\xP@checkspline\xP@splinemultsolid\xP@trblstroke}
\newcommand*\xP@doublestroke{\xydashh@/2,-\xydashh@/2}
\newcommand*\xP@trblstroke{\xydashh@,\z@,-\xydashh@}
\newcommand*\xP@checkspline[1]{\readsplineparams@
\let\next@\@gobble
\ifdim\dimen5<\dimen7
\xP@preparespline
\ifdim\@tempdimb>\z@
\ifdim\@tempdimb<2\dimexpr\xP@preclw\relax
\let\next@\xP@splinemultsolid
\else
\let\next@#1\fi
\fi
\fi
\next@
}
\newcommand*\xP@splinemultsolid[1]{{\xP@inibigdim
\@temptokena{}\xP@setsolidpat
\@for\@tempa:={#1}\do{\xP@paintsolid\z@\xP@bigdim}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintsolid[2]{{\xP@savepts
\xP@a#1\relax
\xP@c#2\relax
\xP@movetotrue
\xP@paintsolid@
\xdef\@gtempa{\the\@temptokena}}\@temptokena\expandafter{\@gtempa}}
\newcommand*\xP@paintsolid@{\xP@b\xP@c
\xP@off\dimexpr\@tempa\relax
\ifdim\xP@off=\z@
\xP@shaveprec\xP@a\xP@c
\else
\loop
\xP@restorepts
\xP@offsetsegment
\xP@testoffset
\unless\ifxP@offsetok
\xP@b\dimexpr\xP@a+(\xP@b-\xP@a)*7/10\relax
\repeat
\fi
\xP@append\@temptokena{\ifxP@moveto\xP@coor\X@p\Y@p m \fi
\xP@coor\L@c\U@c\xP@coor\R@c\D@c\xP@coor\X@c\Y@c c }\xP@movetofalse
\ifdim\xP@b<\xP@c\relax
\xP@a\xP@b
\expandafter\xP@paintsolid@
\fi
}
\@ifdefinable\ifxP@moveto\relax
\@ifdefinable\xP@movetotrue\relax
\@ifdefinable\xP@movetofalse\relax
\newif\ifxP@moveto
\newcommand*\xP@savepts{\xP@xa\X@p
\xP@ya\Y@p
\xP@xb\L@c
\xP@yb\U@c
\xP@xc\R@c
\xP@yc\D@c
\xP@xd\X@c
\xP@yd\Y@c
}
\newcommand*\xP@restorepts{\X@p\xP@xa
\Y@p\xP@ya
\L@c\xP@xb
\U@c\xP@yb
\R@c\xP@xc
\D@c\xP@yc
\X@c\xP@xd
\Y@c\xP@yd
}
\@ifdefinable\xP@tmx\relax
\@ifdefinable\xP@tmy\relax
\newcommand*\xP@Tmxy{*\xP@Tmx/\xP@Tmy}
\newcommand*\xP@Tmyx{*\xP@Tmy/\xP@Tmx}
\newcommand*\xP@Tmzero{*\z@}
\newcommand*\xP@offsetsegment{{\xP@tangentvec\xP@a
\xP@xa\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\xP@a/8+\d@Y*\xP@off/\@tempdimb\relax
\xP@ya\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\xP@a/8-\d@X*\xP@off/\@tempdimb\relax
\xP@scaleT
\xP@Tax\d@X
\xP@Tay\d@Y
\xP@E\@tempdimb
\xP@tangentvec\xP@b
\xP@xd\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\xP@b/8+\d@Y*\xP@off/\@tempdimb\relax
\xP@yd\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\xP@b/8-\d@X*\xP@off/\@tempdimb\relax
\xP@scaleT
\xP@Tdx-\d@X
\xP@Tdy-\d@Y
\xP@F\@tempdimb
\xP@M\z@
\xP@Max\xP@M\xP@Tdx
\xP@Max\xP@M\xP@Tdy
\xP@L\dimexpr\xP@Tax*\xP@Tdx/\xP@M+\xP@Tay*\xP@Tdy/\xP@M\relax
\xP@tm\dimexpr(\xP@a+\xP@b)/2\relax
\ifdim\xP@L>\dimexpr\xP@E*\xP@F/\xP@M*49/50\relax
\d@X-\dimexpr\xP@Tay+\xP@Tdy\relax
\d@Y\dimexpr\xP@Tax+\xP@Tdx\relax
\xP@veclen
\xP@A\dimexpr\X@c-\X@p\relax
\xP@B\dimexpr\Y@c-\Y@p\relax
\xP@M\z@
\xP@Max\xP@M\xP@A
\xP@Max\xP@M\xP@B
\ifdim\xP@M=\z@
\xP@A\dimexpr\R@c-\L@c\relax
\xP@B\dimexpr\D@c-\U@c\relax
\xP@Max\xP@M\xP@A
\xP@Max\xP@M\xP@B
\fi
\xP@M\dimexpr\d@X*\xP@A/\xP@M+\d@Y*\xP@B/\xP@M\relax
\ifdim\xP@M<\z@
\multiply\d@X\m@ne
\multiply\d@Y\m@ne
\fi
\else
\xP@tangentvec\xP@tm
\fi
\xP@xm\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\xP@tm+8\d@Y*\xP@off/\@tempdimb\relax
\xP@ym\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\xP@tm-8\d@X*\xP@off/\@tempdimb\relax
\xP@Tmx\d@X
\xP@Tmy\d@Y
\xP@ifabsless\xP@Tmy\xP@Tmx
\let\xP@tmy\xP@Tmyx
\let\xP@tmx\@empty
\else
\ifdim\xP@Tmy=\z@
\let\xP@tmx\xP@Tmzero
\let\xP@tmy\xP@Tmzero
\else
\let\xP@tmy\@empty
\let\xP@tmx\xP@Tmxy
\fi
\fi
\xP@fa\p@
\xP@fd\p@
\xP@tm\p@
\count@\z@
\loop
\xP@offsetpoints
\@tempswafalse
\ifnum10>\count@
\xP@objfun\xP@oldobj
\ifdim\xP@oldobj>\xP@maxobjfun\relax\@tempswatrue\fi
\fi
\if@tempswa
\xP@offsetloop
\repeat
\xdef\@gtempa{\X@p\the\xP@xa\Y@p\the\xP@ya
\L@c\the\xP@xb\U@c\the\xP@yb\R@c\the\xP@xc\D@c\the\xP@yc
\X@c\the\xP@xd\Y@c\the\xP@yd\relax}}\@gtempa
}
\newcommand*\xP@scaleT{\xP@B6.28\xP@off
\xP@abs\xP@B
\xP@C\dimexpr\d@X*\xP@B/\@tempdimb\relax
\xP@D\dimexpr\d@Y*\xP@B/\@tempdimb\relax
\xP@A\dimexpr\xP@b-\xP@a\relax
\d@X\dimexpr\xP@C+\d@X*\xP@A/\xP@bigdim\relax
\d@Y\dimexpr\xP@D+\d@Y*\xP@A/\xP@bigdim\relax
\@tempdimb\dimexpr\xP@B+\@tempdimb*\xP@A/\xP@bigdim\relax
}
\newcommand*\xP@offsetloop{\xP@C\dimexpr\xP@C/2\relax
\xP@G\dimexpr\xP@G/2\relax
\xP@ta\dimexpr2\p@-\xP@tm\relax
\xP@tb\dimexpr\xP@tm*\xP@ta/\p@\relax
\xP@A\dimexpr\xP@Tax*\xP@tb/\p@*\xP@ta/\p@\relax
\xP@B\dimexpr\xP@Tdx*\xP@tb/\p@*\xP@tm/\p@\relax
\xP@E\dimexpr\xP@Tay*\xP@tb/\p@*\xP@ta/\p@\relax
\xP@F\dimexpr\xP@Tdy*\xP@tb/\p@*\xP@tm/\p@\relax
\xP@tb\dimexpr2\p@-3\xP@tm\relax
\xP@tc\dimexpr\xP@tb+2\p@\relax
\xP@I\dimexpr(2\xP@Tay\xP@tmx-2\xP@Tax\xP@tmy)*\xP@tb/\p@*\xP@ta/\p@\relax
\xP@J\dimexpr(2\xP@Tdy\xP@tmx-2\xP@Tdx\xP@tmy)*\xP@tc/\p@*\xP@tm/\p@\relax
\xP@K\dimexpr((\xP@yd-\xP@ya+(\xP@yb-\xP@yc)*3)
*\xP@tm/\p@+(\xP@yc-2\xP@yb+\xP@ya)*2)*12\xP@tmx
-((\xP@xd-\xP@xa+(\xP@xb-\xP@xc)*3)
*\xP@tm/\p@+(\xP@xc-2\xP@xb+\xP@xa)*2)*12\xP@tmy\relax
\xP@solvelinearsystem
\ifxP@validsol
\xP@correctsol
\ifdim\xP@ta=\z@
\ifdim\xP@tb=\z@
\ifdim\xP@tc=\z@
\xP@validsolfalse
\fi\fi\fi
\fi
\ifxP@validsol
\else
\xP@applinsys
\advance\xP@fa-\xP@ta
\advance\xP@fd-\xP@tb
\advance\xP@tm-\xP@tc
\ifdim\xP@tm<\z@\xP@tm\z@\fi
\ifdim\xP@tm>2\p@\xP@tm2\p@\fi
\fi
\advance\count@\@ne
}
\newcommand*\xP@maxsol{3pt}
\newcommand*\xP@correctsol{\xP@M\z@
\xP@Max\xP@M\xP@ta
\xP@Max\xP@M\xP@tb
\xP@Max\xP@M\xP@tc
\ifdim\xP@M>\xP@maxsol
\xP@ta\dimexpr\xP@maxsol*\xP@ta/\xP@M\relax
\xP@tb\dimexpr\xP@maxsol*\xP@tb/\xP@M\relax
\xP@tc\dimexpr\xP@maxsol*\xP@tc/\xP@M\relax
\fi
\advance\xP@fa-\xP@ta
\advance\xP@fd-\xP@tb
\xP@M\xP@tm
\advance\xP@tm-\xP@tc
\ifdim\xP@tm<\z@\xP@tm\z@\fi
\ifdim\xP@tm>2\p@\xP@tm2\p@\fi
{\xP@offsetpoints
\xP@objfun\xP@M
\expandafter}\ifdim\xP@M>\xP@oldobj
\advance\xP@fa\xP@ta
\advance\xP@fd\xP@tb
\xP@tm\xP@M
\xP@validsolfalse
\fi
}
\newcommand*\xP@objfun[1]{\xP@D\dimexpr\xP@bezierpoly\xP@xa\xP@xb\xP@xc\xP@xd\xP@tm-\xP@xm\relax
\xP@H\dimexpr\xP@bezierpoly\xP@ya\xP@yb\xP@yc\xP@yd\xP@tm-\xP@ym\relax
\xP@C\xP@beziertan\xP@xa\xP@xb\xP@xc\xP@xd\xP@tm
\xP@G\xP@beziertan\xP@ya\xP@yb\xP@yc\xP@yd\xP@tm
\xP@L\dimexpr\xP@G\xP@tmx-\xP@C\xP@tmy\relax
#1\z@
\xP@Max#1\xP@D
\xP@Max#1\xP@H
\xP@Max#1\xP@L
#1\ifdim#1>4843165sp
\maxdimen
\else
\dimexpr\xP@D*\xP@D/\p@+\xP@H*\xP@H/\p@+\xP@L*\xP@L/\p@\relax
\fi
}
\newcommand*\xP@offsetpoints{\xP@xb\dimexpr\xP@xa+\xP@Tax*\xP@fa/196608\relax
\xP@yb\dimexpr\xP@ya+\xP@Tay*\xP@fa/196608\relax
\xP@xc\dimexpr\xP@xd+\xP@Tdx*\xP@fd/196608\relax
\xP@yc\dimexpr\xP@yd+\xP@Tdy*\xP@fd/196608\relax
}
\newcommand*\xP@bezierpoly[5]{\dimexpr(((#4-#1+(#2-#3)*3)*#5/\p@+(#1-2#2+#3)*6)*#5/\p@+(#2-#1)*12)*#5/\p@
+#1*8\relax
}
\newcommand*\xP@precbezierpoly[5]{\dimexpr(((#4-#1+(#2-#3)*3)*2*#5/\xP@bigdim+(#1-2#2+#3)*6)*2*#5/\xP@bigdim
+(#2-#1)*12)*2*#5/\xP@bigdim+#1*8\relax
}
\newcommand*\xP@beziertan[5]{\dimexpr((#4-#1+(#2-#3)*3)*3*#5/32768+(#1-2#2+#3)*24)*#5/\p@+(#2-#1)*24\relax
}
\newcommand*\xP@precbeziertan[5]{\dimexpr((#4-#1+(#2-#3)*3)*#5/\xP@bigdim+(#1-2#2+#3)*2)*#5/\xP@bigdim
+#2-#1\relax
}
\@ifdefinable\xP@varone\relax
\@ifdefinable\xP@vartwo\relax
\@ifdefinable\xP@varthree\relax
\@ifdefinable\ifxP@validsol\relax
\@ifdefinable\xP@validsoltrue\relax
\@ifdefinable\xP@validsolfalse\relax
\newif\ifxP@validsol
\newcommand*\xP@solvelinearsystem{{\xP@scalerow\xP@A\xP@B\xP@C\xP@D
\xP@scalerow\xP@E\xP@F\xP@G\xP@H
\xP@scalerow\xP@I\xP@J\xP@K\xP@L
\xP@scalecol\xP@A\xP@E\xP@I\xP@scaleone
\xP@scalecol\xP@B\xP@F\xP@J\xP@scaletwo
\xP@scalecol\xP@C\xP@G\xP@K\xP@scalethree
\let\xP@varone\xP@ta
\let\xP@vartwo\xP@tb
\let\xP@varthree\xP@tc
\count@\m@ne
\@tempcnta\m@ne
\xP@ifabsless\xP@A\xP@B\@tempcnta\z@\xP@M\xP@B
\else\xP@M\xP@A\fi
\xP@ifabsless\xP@M\xP@C\@tempcnta\@ne\xP@M\xP@C\fi
\xP@ifabsless\xP@M\xP@E\@tempcnta\m@ne\count@\z@\xP@M\xP@E\fi
\xP@ifabsless\xP@M\xP@F\@tempcnta\z@\count@\z@\xP@M\xP@F\fi
\xP@ifabsless\xP@M\xP@G\@tempcnta\@ne\count@\z@\xP@M\xP@G\fi
\xP@ifabsless\xP@M\xP@I\@tempcnta\m@ne\count@\@ne\xP@M\xP@I\fi
\xP@ifabsless\xP@M\xP@J\@tempcnta\z@\count@\@ne\xP@M\xP@J\fi
\xP@ifabsless\xP@M\xP@K\@tempcnta\@ne\count@\@ne\fi
\ifcase\count@
\xP@swapdim\xP@A\xP@E
\xP@swapdim\xP@B\xP@F
\xP@swapdim\xP@C\xP@G
\xP@swapdim\xP@D\xP@H
\or
\xP@swapdim\xP@A\xP@I
\xP@swapdim\xP@B\xP@J
\xP@swapdim\xP@C\xP@K
\xP@swapdim\xP@D\xP@L
\fi
\ifcase\@tempcnta
\xP@swapdim\xP@A\xP@B
\xP@swapdim\xP@E\xP@F
\xP@swapdim\xP@I\xP@J
\let\xP@varone\xP@tb
\let\xP@vartwo\xP@ta
\xP@swapnum\xP@scaleone\xP@scaletwo
\or
\xP@swapdim\xP@A\xP@C
\xP@swapdim\xP@E\xP@G
\xP@swapdim\xP@I\xP@K
\let\xP@varone\xP@tc
\let\xP@varthree\xP@ta
\xP@swapnum\xP@scaleone\xP@scalethree
\fi
\multiply\xP@E\m@ne
\multiply\xP@I\m@ne
\ifdim\xP@A=\z@
\else
\advance\xP@F\dimexpr\xP@B*\xP@E/\xP@A\relax
\advance\xP@G\dimexpr\xP@C*\xP@E/\xP@A\relax
\advance\xP@H\dimexpr\xP@D*\xP@E/\xP@A\relax
\advance\xP@J\dimexpr\xP@B*\xP@I/\xP@A\relax
\advance\xP@K\dimexpr\xP@C*\xP@I/\xP@A\relax
\advance\xP@L\dimexpr\xP@D*\xP@I/\xP@A\relax
\fi
\count@\m@ne
\xP@ifabsless\xP@F\xP@G\@tempcnta\z@\xP@M\xP@G
\else\@tempcnta\m@ne\xP@M\xP@F\fi
\xP@ifabsless\xP@M\xP@J\@tempcnta\m@ne\count@\z@\xP@M\xP@J\fi
\xP@ifabsless\xP@M\xP@K\@tempcnta\z@\count@\z@\fi
\ifnum\count@=\z@
\xP@swapdim\xP@F\xP@J
\xP@swapdim\xP@G\xP@K
\xP@swapdim\xP@H\xP@L
\fi
\ifnum\@tempcnta=\z@
\xP@swapdim\xP@B\xP@C
\xP@swapdim\xP@F\xP@G
\xP@swapdim\xP@J\xP@K
\let\@tempa\xP@varthree
\let\xP@varthree\xP@vartwo
\let\xP@vartwo\@tempa
\xP@swapnum\xP@scaletwo\xP@scalethree
\fi
\ifdim\xP@F=\z@
\else
\advance\xP@K\dimexpr-\xP@G*\xP@J/\xP@F\relax
\advance\xP@L\dimexpr-\xP@H*\xP@J/\xP@F\relax
\fi
\xP@ifabsless{\dimexpr\xP@L/60\relax}{\dimexpr\xP@K/\xP@scalethree\relax}\xP@validsoltrue
\xP@varthree\dimexpr\xP@L*(\xP@scalethree*\p@)/\xP@K\relax
\else
\xP@validsolfalse
\fi
\xP@checkabs{\xP@H/8191}{\xP@F/\xP@scaletwo}\xP@checkabs{\xP@G/\xP@scalethree/136}{\xP@F/\xP@scaletwo}\ifxP@validsol
\xP@vartwo\dimexpr\xP@H*(\xP@scaletwo*\p@)/\xP@F
-\xP@varthree*\xP@scaletwo/\xP@scalethree*\xP@G/\xP@F\relax
\xP@checkabs\xP@vartwo{60pt}\fi
\xP@checkabs{\xP@D/5461}{\xP@A/\xP@scaleone}\xP@checkabs{\xP@B/\xP@scaletwo/91}{\xP@A/\xP@scaleone}\xP@checkabs{\xP@C/\xP@scalethree/91}{\xP@A/\xP@scaleone}\ifxP@validsol
\xP@varone\dimexpr\xP@D*(\xP@scaleone*\p@)/\xP@A
-\xP@vartwo*\xP@scaleone/\xP@scaletwo*\xP@B/\xP@A
-\xP@varthree*\xP@scaleone/\xP@scalethree*\xP@C/\xP@A\relax
\xP@checkabs\xP@varone{60pt}\fi
\xdef\@gtempa{\ifxP@validsol
\xP@ta\the\xP@ta\relax
\xP@tb\the\xP@tb\relax
\xP@tc\the\xP@tc\relax
\noexpand\xP@validsoltrue
\else
\noexpand\xP@validsolfalse
\fi
}}\@gtempa
}
\newcommand*\xP@scalerow[4]{\xP@M\z@
\xP@Max\xP@M#1\xP@Max\xP@M#2\xP@Max\xP@M#3\xP@Max\xP@M#4\count@134217727
\loop
\divide\xP@M\tw@
\ifdim\xP@M>\z@
\divide\count@\tw@
\repeat
\advance\count@\@ne
\multiply#1\count@
\multiply#2\count@
\multiply#3\count@
\multiply#4\count@
}
\newcommand*\xP@scalecol[4]{\xP@M\z@
\xP@Max\xP@M#1\xP@Max\xP@M#2\xP@Max\xP@M#3#416777215
\loop
\divide\xP@M\tw@
\ifdim\xP@M>\z@
\divide#4\tw@
\repeat
\advance#4\@ne
\multiply#1#4\multiply#2#4\multiply#3#4}
\newcommand*\xP@checkabs[2]{\xP@ifabsless{\dimexpr#1\relax}{\dimexpr#2\relax}\else\xP@validsolfalse\fi}
\newcommand*\xP@applinsys{{\xP@applinsys@
\xP@ta\xP@dta
\xP@tb\xP@dtb
\xP@tc\xP@dtc
\xP@checkapp
\if@tempswa
\xP@modobj
\xP@applinsys@
\xP@checkapp
\if@tempswa
\xP@modsol
\xP@modobj
\xP@applinsys@
\xP@modsol
\fi
\fi
\xdef\@gtempa{\xP@ta\the\xP@ta\relax
\xP@tb\the\xP@tb\relax
\xP@tc\the\xP@tc\relax
}}\@gtempa
}
\newcommand*\xP@checkapp{\@tempswatrue
\ifdim\xP@dta=\z@
\ifdim\xP@dtb=\z@
\ifdim\xP@dtc=\z@
\@tempswafalse
\fi\fi\fi
}
\newcommand*\xP@modobj{\advance\xP@D
\dimexpr-\xP@A*\xP@dta/\p@-\xP@B*\xP@dtb/\p@-\xP@C*\xP@dtc/\p@\relax
\advance\xP@H
\dimexpr-\xP@E*\xP@dta/\p@-\xP@F*\xP@dtb/\p@-\xP@G*\xP@dtc/\p@\relax
\advance\xP@L
\dimexpr-\xP@I*\xP@dta/\p@-\xP@J*\xP@dtb/\p@-\xP@K*\xP@dtc/\p@\relax
}
\newcommand*\xP@modsol{\advance\xP@ta\xP@dta
\advance\xP@tb\xP@dtb
\advance\xP@tc\xP@dtc
}
\newcommand*\xP@applinsys@{{\xP@sa\z@
\xP@Max\xP@sa\xP@A
\xP@Max\xP@sa\xP@B
\xP@Max\xP@sa\xP@C
\xP@Max\xP@sa\xP@E
\xP@Max\xP@sa\xP@F
\xP@Max\xP@sa\xP@G
\xP@Max\xP@sa\xP@I
\xP@Max\xP@sa\xP@J
\xP@Max\xP@sa\xP@K
\xP@sa\ifdim\xP@sa<5460pt\thr@@\xP@sa\else\maxdimen\fi
\xP@sb\z@
\xP@Max\xP@sb\xP@D
\xP@Max\xP@sb\xP@H
\xP@Max\xP@sb\xP@L
\ifdim\xP@sb>\z@
\xP@D\dimexpr\xP@D*\maxdimen/\xP@sb\relax
\xP@H\dimexpr\xP@H*\maxdimen/\xP@sb\relax
\xP@L\dimexpr\xP@L*\maxdimen/\xP@sb\relax
\fi
\xP@Aba\dimexpr\xP@A*\xP@D/\xP@sa+\xP@E*\xP@H/\xP@sa+\xP@I*\xP@L/\xP@sa\relax
\xP@Abb\dimexpr\xP@B*\xP@D/\xP@sa+\xP@F*\xP@H/\xP@sa+\xP@J*\xP@L/\xP@sa\relax
\xP@Abc\dimexpr\xP@C*\xP@D/\xP@sa+\xP@G*\xP@H/\xP@sa+\xP@K*\xP@L/\xP@sa\relax
\xP@AAba\dimexpr\xP@A*\xP@Aba/\xP@sa+\xP@B*\xP@Abb/\xP@sa
+\xP@C*\xP@Abc/\xP@sa\relax
\xP@AAbb\dimexpr\xP@E*\xP@Aba/\xP@sa+\xP@F*\xP@Abb/\xP@sa
+\xP@G*\xP@Abc/\xP@sa\relax
\xP@AAbc\dimexpr\xP@I*\xP@Aba/\xP@sa+\xP@J*\xP@Abb/\xP@sa
+\xP@K*\xP@Abc/\xP@sa\relax
\xP@sc\z@
\xP@Max\xP@sc\xP@Aba
\xP@Max\xP@sc\xP@Abb
\xP@Max\xP@sc\xP@Abc
\xP@Max\xP@sc\xP@AAba
\xP@Max\xP@sc\xP@AAbb
\xP@Max\xP@sc\xP@AAbc
\ifdim\xP@sc=\z@
\xP@AAb\z@
\else
\xP@Ab\dimexpr\xP@Aba*\xP@bigdim/\xP@sc*\xP@Aba/\xP@sc
+\xP@Abb*\xP@bigdim/\xP@sc*\xP@Abb/\xP@sc
+\xP@Abc*\xP@bigdim/\xP@sc*\xP@Abc/\xP@sc
\relax
\xP@AAb\dimexpr\xP@AAba*\xP@bigdim/\xP@sc*\xP@AAba/\xP@sc
+\xP@AAbb*\xP@bigdim/\xP@sc*\xP@AAbb/\xP@sc
+\xP@AAbc*\xP@bigdim/\xP@sc*\xP@AAbc/\xP@sc
\relax
\fi
\xdef\@gtempa{\ifdim\xP@AAb=\z@
\xP@dta\z@
\xP@dtb\z@
\xP@dtc\z@
\else
\xP@dta\the\dimexpr\xP@Aba*\xP@sb/\xP@sa*\p@/\xP@AAb*\xP@Ab/\maxdimen
\relax
\xP@dtb\the\dimexpr\xP@Abb*\xP@sb/\xP@sa*\p@/\xP@AAb*\xP@Ab/\maxdimen
\relax
\xP@dtc\the\dimexpr\xP@Abc*\xP@sb/\xP@sa*\p@/\xP@AAb*\xP@Ab/\maxdimen
\relax
\fi
}}\@gtempa
}
\@ifdefinable\ifxP@offsetok\relax
\@ifdefinable\xP@offsetoktrue\relax
\@ifdefinable\xP@offsetokfalse\relax
\newif\ifxP@offsetok
\newcommand*\xP@maxdev{.1pt}
\newcommand*\xP@maxobjfun{.005pt}
\newcommand*\xP@testoffset{{\gdef\xP@afteroffsetok{\xP@offsetoktrue}\def\xP@offsetokif{\ifdim\xP@ti<1.85pt}\xP@ti.1pt
\loop
\xP@tip\dimexpr\xP@a+(\xP@b-\xP@a)*\xP@ti/131072\relax
\L@p\xP@precbezierpoly\xP@xa\xP@xb\xP@xc\xP@xd\xP@tip
\U@p\xP@precbezierpoly\xP@ya\xP@yb\xP@yc\xP@yd\xP@tip
\xP@valA\dimexpr\xP@bezierpoly\X@p\L@c\R@c\X@c\xP@ti-\L@p\relax
\xP@valB\dimexpr\xP@bezierpoly\Y@p\U@c\D@c\Y@c\xP@ti-\U@p\relax
\d@X3\xP@precbeziertan\xP@xa\xP@xb\xP@xc\xP@xd\xP@tip
\d@Y3\xP@precbeziertan\xP@ya\xP@yb\xP@yc\xP@yd\xP@tip
\xP@veclen
\@tempdimc\dimexpr(\xP@b-\xP@a)*\@tempdimb/\xP@bigdim\relax
\xP@abs\@tempdimc
\ifdim.01pt<\@tempdimc
\xP@devA\dimexpr\xP@valA*\d@X/\@tempdimb+\xP@valB*\d@Y/\@tempdimb\relax
\xP@devB\dimexpr\xP@valA*\d@Y/\@tempdimb-\xP@valB*\d@X/\@tempdimb-8\xP@off
\relax
\xP@abs\xP@devA
\xP@abs\xP@devB
\@tempdima\dimexpr\xP@devA+\xP@devB\relax
\else
\ifdim\@tempdimc=\z@
\@tempdima\z@
\else
{\d@X\xP@valA
\d@Y\xP@valB
\xP@veclen@
\global\dimen@i\@tempdimb
}\@tempdima\dimen@i
\advance\@tempdima\ifdim\xP@off>\z@-\fi8\xP@off
\xP@abs\@tempdima
\fi
\fi
\ifdim\@tempdima>\xP@maxdev
\divide\L@p-8\relax
\divide\U@p-8\relax
{\xP@transformcoor\X@p\Y@p
\xP@transformcoor\L@c\U@c
\xP@transformcoor\R@c\D@c
\xP@transformcoor\X@c\Y@c
\xP@findzero
}\fi
\xP@offsetokif
\advance\xP@ti.1pt
\repeat
\expandafter}\xP@afteroffsetok
}
\newcommand*\xP@afteroffsetok{}
\newcommand*\xP@offsetokif{}
\newcommand*\xP@transformcoor[2]{\advance#1\L@p
\advance#2\U@p
\@tempdima\dimexpr#1*\d@X/\@tempdimb+#2*\d@Y/\@tempdimb\relax
#2\dimexpr#2*\d@X/\@tempdimb-#1*\d@Y/\@tempdimb\relax
#1\@tempdima
}
\newcommand*\xP@findzero{\xP@setleftvalue{.05}\xP@setrightvalue{.05}\ifdim\xP@valB<\z@\xP@reversecoeff\fi
\ifdim\xP@valA>\z@
\@tempswatrue
\@for\@tempa:={.1,.15,.2,.25,.35,.5,1.1}\do{\if@tempswa
\xP@setleftvalue\@tempa
\ifdim\xP@valA<\z@\@tempswafalse\fi
\if@tempswa
\xP@setrightvalue\@tempa
\ifdim\xP@valB<\z@
\@tempswafalse
\xP@reversecoeff
\fi
\fi
\fi
}\if@tempswa
\L@p\xP@ti
\xP@valA\xP@bezierpoly\X@p\L@c\R@c\X@c\L@p
\ifdim\xP@valA<\z@
\xP@setrightvalue{.05}\else
\U@p\L@p
\xP@valB\xP@valA
\fi
\fi
\fi
\loop
\ifnum\numexpr\U@p-\L@p\relax>\@ne
\xP@ti\dimexpr(\L@p+\U@p)/2\relax
\xP@devA\xP@bezierpoly\X@p\L@c\R@c\X@c\xP@ti
\ifdim\xP@devA>\z@
\U@p\xP@ti
\xP@valB\xP@devA
\else
\L@p\xP@ti
\xP@valA\xP@devA
\fi
\repeat
\xP@ifabsless\xP@valB\xP@valA
\L@p\U@p
\xP@valA\xP@valB
\fi
\xP@valB\dimexpr\xP@bezierpoly\Y@p\U@c\D@c\Y@c\L@p+8\xP@off\relax
\xP@abs\xP@valA
\xP@abs\xP@valB
\ifdim\dimexpr\xP@valA+\xP@valB\relax>\xP@maxdev\relax
\xP@failed
\fi
}
\newcommand*\xP@failed{\global\let\xP@offsetokif\iffalse
\gdef\xP@afteroffsetok{\xP@offsetokfalse}}
\newcommand*\xP@reversecoeff{\multiply\X@p\m@ne
\multiply\L@c\m@ne
\multiply\R@c\m@ne
\multiply\X@c\m@ne
\multiply\xP@valA\m@ne
\multiply\xP@valB\m@ne
}
\newcommand*\xP@setleftvalue[1]{\L@p\dimexpr\xP@ti-#1\p@\relax
\ifdim\L@p<-.1pt\L@p-.1pt\fi
\xP@valA\xP@bezierpoly\X@p\L@c\R@c\X@c\L@p
}
\newcommand*\xP@setrightvalue[1]{\U@p\dimexpr\xP@ti+#1\p@\relax
\ifdim\U@p>2.1\p@\U@p2.1\p@\fi
\xP@valB\xP@bezierpoly\X@p\L@c\R@c\X@c\U@p
}
\newcommand*\xP@splinedbldashed{\xP@checkspline\xP@splinemultdashed\xP@doublestroke}
\newcommand*\xP@splinetrbldashed{\xP@checkspline\xP@splinemultdashed\xP@trblstroke}
\newcommand*\xP@splinemultdashed[1]{\xP@testcont\xP@dashmacro
\@tempcnta
\ifxP@splinecont
\numexpr2*((\@tempdimb-\xydashl@/3)/(2*\xydashl@))\relax
\else
\numexpr2*((\@tempdimb+\xydashl@)/(2*\xydashl@))-1\relax
\fi
\ifnum\@tempcnta>\@ne
\xP@splinemultdashed@#1\else
\ifnum\@tempcnta=\@ne
\xP@splinemultsolid#1
\else
\xP@savec
\fi
\fi
\global\let\xP@lastpattern\xP@dashmacro
}
\newcommand*\xP@splinemultdashed@[1]{{\xP@inibigdim
\@tempdima\dimexpr\@tempdimb/\@tempcnta\relax
\xP@temppar\z@
\toks@{}\xP@savec
\ifodd\@tempcnta
\else
\xP@slide
\fi
\@tempcnta\z@
\loop
\advance\@tempcnta\@ne
\xP@append\toks@{\ifodd\@tempcnta\noexpand\xP@paintdash\fi
{\the\xP@temppar}}\xP@oldpar\xP@temppar
\xP@slide
\ifdim\xP@temppar<\xP@bigdim
\repeat
\xP@lastpar
\ifodd\@tempcnta
\xP@temppar
\xP@append\toks@{{\the\xP@temppar}}\else
\xP@oldpar
\fi
\@temptokena{}\xP@setsolidpat
\global\let\xP@lastpattern\xP@dashmacro
\@for\@tempa:={#1}\do{\the\toks@}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintdash[2]{\xP@paintsolid{\dimexpr#1*\xP@bigdim/\xP@lastpar\relax}{\dimexpr#2*\xP@bigdim/\xP@lastpar\relax}}
\xP@hook{curve}{splinedbldotted@}
\newcommand*\xP@splinedbldotted@{\let\xP@normalmult\@ne
\xP@checkspline\xP@splinemultdotted\xP@doublestroke}
\newcommand*\xP@splinetrbldotted{\let\xP@normalmult\tw@
\xP@checkspline\xP@splinemultdotted\xP@trblstroke}
\newcommand*\xP@multidottedpat{\def\xP@pattern{0 J [\xP@coor\xP@preclw{\xydashh@-\xP@preclw}]0 d}\global\let\xP@lastpattern\xP@dotmacro
}
\@ifdefinable\xP@normalmult\relax
\newcommand\xP@splinemultdotted[1]{{\xP@inibigdim
\xP@temppar\z@
\xP@testcont\xP@dotmacro
\ifxP@splinecont
\@tempdimc\dimexpr\@tempdimb/(\@tempdimb/131072+1)\relax
\@tempdima\dimexpr\@tempdimc-\xP@preclw/2\relax
\xP@slide
\@tempdima\@tempdimc
\else
\@tempdima\dimexpr\xP@preclw/2\relax
\xP@slide
\@tempdima\dimexpr\@tempdimb-\xP@preclw\relax
\ifdim\@tempdima<\z@\@tempdima\z@\fi
\@tempdima\dimexpr\@tempdima/(\@tempdima/131072+1)\relax
\fi
\xP@savec
\toks@{}\ifdim\xP@temppar<\xP@bigdim
\loop
\xP@append\toks@{\noexpand\xP@paintdot{\the\xP@temppar}}\xP@oldpar\xP@temppar
\xP@slide
\ifdim\xP@temppar<\xP@bigdim
\repeat
\xP@velocity\xP@bigdim\xP@tempvel
\ifdim
\ifdim\xP@preclw<\xP@tempvel
\dimexpr2\xP@bigdim-\xP@oldpar-\xP@preclw*\xP@bigdim/\xP@tempvel\relax
\else
-\maxdimen
\fi<\xP@temppar
\xP@temppar\xP@oldpar
\else
\xP@append\toks@{\noexpand\xP@paintdot{\the\xP@temppar}}\fi
\@tempdima\dimexpr\xP@preclw/2\relax
\xP@slide
\xP@lastpar\xP@temppar
\@temptokena{}\the\toks@
\xP@multidottedpat
\xP@stroke{\the\@temptokena}\else
\global\let\xP@lastpattern\@empty
\fi
}}
\newcommand*\xP@slide{{\xP@slide@
\global\dimen@i\xP@temppar
}\xP@temppar\dimen@i
}
\newcommand*\xP@slide@{\xP@velocity\xP@temppar\xP@tempvel
\@tempdimc\dimexpr\xP@bigdim*\@tempdima/\@tempdimb\relax
\count@\z@
\@tempswatrue
\loop
\xP@velocity{\xP@temppar+\@tempdimc}\xP@tempvel@
\ifdim\dimexpr\@tempdima*4/13\relax>\xP@tempvel@
\@tempswafalse
\else
\xP@parinc\dimexpr\@tempdima*\xP@bigdim/\xP@tempvel@
-(\xP@tempvel+\xP@tempvel@)/2*\@tempdimc/\xP@tempvel@\relax
\advance\@tempdimc\xP@parinc
\ifdim\@tempdimc>.12\xP@bigdim
\@tempswafalse
\else
\ifdim\xP@parinc=\z@
\@tempswafalse
\else
\ifnum\count@=9\relax
\@tempswafalse
\fi
\fi
\fi
\fi
\if@tempswa
\advance\count@\@ne
\repeat
\ifdim\xP@temppar<5461pt
\ifdim\@tempdimc>.1\xP@bigdim
\@tempswatrue
\fi
\fi
\if@tempswa
{\dimen5\xP@temppar
\advance\xP@temppar.1\xP@bigdim
\ifdim\xP@temppar>5461pt\xP@temppar5461pt\fi
\dimen7\xP@temppar
\xP@shaveprec{\dimen5}{\dimen7}\xP@bezierlength
\global\dimen@i\dimexpr\@tempdima-\@tempdimb\relax
\global\dimen3\xP@temppar
}\@tempdima\dimen@i
\xP@temppar\dimen3\relax
\expandafter\xP@slide@
\else
\advance\xP@temppar\@tempdimc
\fi
}
\newcommand*\xP@paintdot[1]{\@tempdima\dimexpr#1*\xP@bigdim/\xP@lastpar\relax
\xP@tangent
\xP@posX\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\@tempdima/8\relax
\xP@posY\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\@tempdima/8\relax
\@tempdima\dimexpr(\xydashh@+\xP@preclw/\xP@normalmult)/2\relax
\L@p\dimexpr\d@Y*\@tempdima/\@tempdimb\relax
\U@p\dimexpr-\d@X*\@tempdima/\@tempdimb\relax
\xP@append\@temptokena{\xP@coor{\xP@posX+\L@p*\xP@normalmult}{\xP@posY+\U@p*\xP@normalmult}m \xP@coor{\xP@posX-\L@p*(\xP@normalmult+\@ne)}{\xP@posY-\U@p*(\xP@normalmult+\@ne)}l }}
\newcommand*\xP@splinesquiggled{\xP@checkspline\xP@splinesquiggled@\z@}
\newcommand*\xP@splinedblsquiggled{\xP@checkspline\xP@splinesquiggled@\xP@doublestroke}
\newcommand*\xP@splinetrblsquiggled{\xP@checkspline\xP@splinesquiggled@\xP@trblstroke}
\newcommand*\xP@splinesquiggled@[1]{{\xP@inibigdim
\xP@testcont\xP@oddsquigglemacro
\ifxP@splinecont
\def\xP@squigsign{-}\else
\let\xP@squigsign\@empty
\fi
\xP@savec
\@tempcnta=\numexpr\@tempdimb/\xybsqll@\relax
\ifnum\@tempcnta<\tw@\@tempcnta\tw@\fi
\multiply\@tempcnta\tw@
\@tempdima\dimexpr\@tempdimb/\@tempcnta\relax
\xP@squiglen\@tempdima
\xP@temppar\z@
\toks@{}\@tempcnta\z@
\loop
\advance\@tempcnta\@ne
\xP@append\toks@{\noexpand\xP@paintsquiggle{\the\xP@temppar}}\xP@oldpar\xP@temppar
\xP@slide
\ifdim\xP@temppar<\xP@bigdim
\repeat
\xP@lastpar
\ifodd\@tempcnta
\xP@oldpar
\advance\@tempcnta\m@ne
\else
\xP@temppar
\xP@append\toks@{\noexpand\xP@paintsquiggle{\the\xP@temppar}}\fi
\@temptokena{}\xP@setsolidpat
\global\expandafter\let\expandafter\xP@lastpattern
\ifodd\numexpr\@tempcnta/2\if\xP@squigsign-+1\fi\relax
\xP@oddsquigglemacro
\else
\xP@evensquigglemacro
\fi
\@for\@tempa:={#1}\do{\let\xP@dosquiggle\xP@dosquiggle@
\count@\z@
\the\toks@
}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintsquiggle[1]{\xP@squigglevectors{#1}\xP@dosquiggle
\ifnum\count@=\thr@@\relax\count@\z@\else\advance\count@\@ne\fi
}
\newcommand*\xP@squigglevectors[1]{\@tempdima\dimexpr#1*\xP@bigdim/\xP@lastpar\relax
\xP@tangent
\xP@posX\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\@tempdima/8-\d@Y*(\@tempa)/\@tempdimb\relax
\xP@posY\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\@tempdima/8+\d@X*(\@tempa)/\@tempdimb\relax
\L@p\dimexpr\d@X*\xP@squiglen/\@tempdimb\relax
\U@p\dimexpr\d@Y*\xP@squiglen/\@tempdimb\relax
\R@p\dimexpr\L@p*543339720/1311738121\relax
\D@p\dimexpr\U@p*543339720/1311738121\relax
\X@min\dimexpr\L@p*362911648/967576667\relax
\Y@min\dimexpr\U@p*362911648/967576667\relax
\X@max\dimexpr(\L@p+\xP@squigsign\U@p)*173517671/654249180\relax
\Y@max\dimexpr(\L@p-\xP@squigsign\U@p)*173517671/654249180\relax
}
\@ifdefinable\xP@dosquiggle@\relax
\newcommand*\xP@dosquiggle@{\edef\next@{\xP@coor{\xP@posX}{\xP@posY}m
\xP@coor{\xP@posX+\Y@max}{\xP@posY+\xP@squigsign\X@max}}\let\xP@dosquiggle\xP@dosquiggle@@
}
\newcommand*\xP@dosquiggle@@{\xP@append\@temptokena{\next@\expandafter\xP@coor
\ifcase\count@
{\xP@posX-\Y@max}{\xP@posY-\xP@squigsign\X@max}\xP@coor\xP@posX\xP@posY
\or
{\xP@posX-\xP@squigsign\D@p-\X@min}{\xP@posY+\xP@squigsign\R@p-\Y@min}\xP@coor{\xP@posX-\xP@squigsign\D@p}{\xP@posY+\xP@squigsign\R@p}\or
{\xP@posX-\X@max}{\xP@posY+\xP@squigsign\Y@max}\xP@coor\xP@posX\xP@posY
\or
{\xP@posX+\xP@squigsign\D@p-\X@min}{\xP@posY-\xP@squigsign\R@p-\Y@min}\xP@coor{\xP@posX+\xP@squigsign\D@p}{\xP@posY-\xP@squigsign\R@p}\fi c }\edef\next@{\expandafter\xP@coor
\ifcase\count@
{\xP@posX+\Y@max}{\xP@posY+\xP@squigsign\X@max}\or
{\xP@posX-\xP@squigsign\D@p+\X@min}{\xP@posY+\xP@squigsign\R@p+\Y@min}\or
{\xP@posX+\X@max}{\xP@posY-\xP@squigsign\Y@max}\or
{\xP@posX+\xP@squigsign\D@p+\X@min}{\xP@posY-\xP@squigsign\R@p+\Y@min}\fi
}}
\newcommand*\xP@splinebrokensquiggled{\xP@checkspline\xP@splinebrokensquiggled@\z@}
\newcommand*\xP@splinebrokendblsquiggled{\xP@checkspline\xP@splinebrokensquiggled@\xP@doublestroke}
\newcommand*\xP@splinebrokentrblsquiggled{\xP@checkspline\xP@splinebrokensquiggled@\xP@trblstroke}
\newcommand*\xP@splinebrokensquiggled@[1]{{\xP@inibigdim
\xP@testcont\xP@brokensquigglemacro
\ifxP@splinecont
\let\xP@squigsign\@firstoftwo
\else
\let\xP@squigsign\@secondoftwo
\fi
\xP@savec
\@tempcnta\numexpr(\@tempdimb\xP@squigsign{}{+2*\xybsqll@})/(4*\xybsqll@)\relax
\ifnum\@tempcnta<\@ne\@tempcnta\@ne\fi
\@tempdima\dimexpr\@tempdimb/(8*\@tempcnta\xP@squigsign{}{-4})\relax
\xP@squiglen\@tempdima
\xP@temppar\z@
\xP@squigsign{\xP@slide\xP@slide\xP@slide\xP@slide}{}\count@\z@
\toks@{}\loop
\xP@append\toks@{\noexpand\xP@paintbrokensquiggle{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@lastpar\xP@temppar
\advance\count@\@ne
\ifnum\count@<\@tempcnta
\xP@slide
\xP@slide
\xP@slide
\xP@slide
\repeat
\@temptokena{}\xP@setsolidpat
\global\let\xP@lastpattern\xP@brokensquigglemacro
\let\xP@squigsign\@empty
\@for\@tempa:={#1}\do{\the\toks@}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintbrokensquiggle[5]{\xP@squigglevectors{#1}\xP@append\@temptokena{\xP@coor\xP@posX\xP@posY m \xP@coor{\xP@posX+\Y@max}{\xP@posY+\X@max}}\xP@squigglevectors{#2}\xP@append\@temptokena{\xP@coor{\xP@posX-\D@p-\X@min}{\xP@posY+\R@p-\Y@min}\xP@coor{\xP@posX-\D@p}{\xP@posY+\R@p}c \xP@coor{\xP@posX-\D@p+\X@min}{\xP@posY+\R@p+\Y@min}}\xP@squigglevectors{#3}\xP@append\@temptokena{\xP@coor{\xP@posX-\X@max}{\xP@posY+\Y@max}\xP@coor\xP@posX\xP@posY c \xP@coor{\xP@posX+\X@max}{\xP@posY-\Y@max}}\xP@squigglevectors{#4}\xP@append\@temptokena{\xP@coor{\xP@posX+\D@p-\X@min}{\xP@posY-\R@p-\Y@min}\xP@coor{\xP@posX+\D@p}{\xP@posY-\R@p}c \xP@coor{\xP@posX+\D@p+\X@min}{\xP@posY-\R@p+\Y@min}}\xP@squigglevectors{#5}\xP@append\@temptokena{\xP@coor{\xP@posX-\Y@max}{\xP@posY-\X@max}\xP@coor\xP@posX\xP@posY c }}
\xyendinput
%%
%% End of file `xypdf-cu.tex'.


==> xypdf-fr.tex <==
%auto-ignore
%%
%% This is file `xypdf-fr.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `frame')
%%
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://www.math.uni-bonn.de/people/muellner>
%% --------------------------------------------------------------------------
%%
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%%
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%%
%% --------------------------------------------------------------------------
%%
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%%
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%%
%% The files with the TeX code are generated by the following command:
%%
%%    latex xypdf.ins
%%
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%%
%% --------------------------------------------------------------------------
%%
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%%
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%%

\xyrequire{curve}\xycatcodes
\expandafter\let\csname xypdf-fr@loaded\endcsname\@empty
\newcommand*\xP@framedrop[1]{\expandafter\frmDrop@\expandafter{\expandafter\def\expandafter\prevEdge@@\expandafter{\prevEdge@@}#1\frmradius@@}}
\xP@hook{frame}{frm{-}}
\expandafter\newcommand\expandafter*\csname xP@frm{-}\endcsname{\xP@framedrop\xP@solidframe
}
\newcommand*\xP@solidframe[1]{\R@#1\relax
\xP@setsolidpat
\let\xP@fillorstroke\xP@stroke
\xP@frameifnotzero\xP@oval
}
\newcommand*\xP@frameifnotzero[1]{\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\DN@{\zeroEdge}\ifx\next@\prevEdge@@
\else
#1\fi
}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\newcommand*\xP@oval{\hskip-\L@c
\lower\D@c\hbox{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\R@\xP@min\R@{.5\dimen@}\R@\xP@min\R@{.5\dimen@ii}\@tempdimb\dimexpr2\dimen@+2\dimen@ii-\R@*696621973/405764219\relax
\ifdim\R@=\z@
\xP@fillorstroke{0 0 \xP@coor\dimen@\dimen@ii re}\else
\def\@tempa{*119763188/267309217}\xP@fillorstroke{\xP@dim\R@0 m \xP@dim{\R@\@tempa}0 0 \xP@dim{\R@\@tempa}0 \xP@dim\R@ c \ifdim2\R@=\dimen@ii\else
0 \xP@dim{\dimen@ii-\R@}l \fi
0 \xP@dim{\dimen@ii-\R@\@tempa}\xP@coor{\R@\@tempa}\dimen@ii
\xP@coor\R@\dimen@ii c \ifdim2\R@=\dimen@\else
\xP@coor{\dimen@-\R@}\dimen@ii l \fi
\xP@coor{\dimen@-\R@\@tempa}\dimen@ii
\xP@coor\dimen@{\dimen@ii-\R@\@tempa}\xP@coor\dimen@{\dimen@ii-\R@} c \ifdim2\R@=\dimen@ii\else
\xP@coor\dimen@\R@ l \fi
\xP@coor\dimen@{\R@\@tempa}\xP@dim{\dimen@-\R@\@tempa}0 \xP@dim{\dimen@-\R@}0 c h}\fi
}}
\xP@hook{frame}{frm[o]{-}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{-}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setsolidpat}}
\newcommand*\xP@ellipseframe[2]{\xP@getradii{#2}\DN@{\zeroEdge}\ifx\next@\prevEdge@@
\else
\def\xP@fillorstroke{#1\xP@stroke}\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\xP@framedellipse}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
\fi
}
\xP@hook{frame}{frm{.}}
\expandafter\newcommand\expandafter*\csname xP@frm{.}\endcsname{\xP@framedrop\xP@rectframedotted
}
\newcommand*\xP@rectframedotted[1]{\R@#1\relax
\xP@frameifnotzero{\ifdim\R@=\z@
\xP@dottedrect
\else
\xP@dottedoval
\fi
}}
\newcommand*\xP@dottedrect{\hskip-\L@c
\lower\D@c\hbox{\dimen@ii\dimexpr\U@c+\D@c\relax
\@tempdimc\dimexpr\xP@preclw/-2\relax
\@tempdimb\dimexpr\L@c+\R@c+\xP@preclw\relax
\xP@contfalse
\xP@setdottedpat
\dimen@\dimexpr\@tempdimb+\@tempdima/2+\@tempdimc\relax
\xP@stroke{\xP@dim\@tempdimc0 m \xP@dim\dimen@0 l \xP@coor\@tempdimc\dimen@ii m \xP@coor\dimen@\dimen@ii l}\let\xP@testcont\xP@alwaysconttrue
\@tempdimb\dimen@ii
\xP@setdottedpat
\dimen@\dimexpr\L@c+\R@c\relax
\advance\dimen@ii\dimexpr\@tempdimc-\@tempdima/2\relax
\multiply\@tempdimc\m@ne
\xP@stroke{0 \xP@dim\@tempdimc m 0 \xP@dim\dimen@ii l \xP@coor\dimen@\@tempdimc m \xP@coor\dimen@\dimen@ii l}}}
\newcommand*\xP@dottedoval{\def\xP@fillorstroke{\xP@setcldottedpat\xP@stroke}\xP@oval
}
\xP@hook{frame}{frm[o]{.}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{.}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldottedpat}}
\xP@hook{frame}{frm{--}}
\expandafter\newcommand\expandafter*\csname xP@frm{--}\endcsname{\xP@framedrop\xP@rectframedashed
}
\newcommand*\xP@rectframedashed[1]{\R@#1\relax
\xP@frameifnotzero{\ifdim\R@=\z@
\xP@dashedrect
\else
\xP@dashedoval
\fi
}}
\newcommand*\xP@dashedrect{\hskip-\L@c
\lower\D@c\hbox{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\@tempdimb\dimen@
\xP@contfalse
\xP@setdashpat
\xP@stroke{0 0 m \xP@dim\dimen@0 l 0 \xP@dim\dimen@ii m \xP@coor\dimen@\dimen@ii l}\@tempdimb\dimen@ii
\xP@setdashpat
\xP@stroke{0 0 m 0 \xP@dim\dimen@ii l \xP@dim\dimen@0 m \xP@coor\dimen@\dimen@ii l}}}
\newcommand*\xP@dashedoval{\def\xP@fillorstroke{\xP@setcldashpat\xP@stroke}\xP@oval
}
\xP@hook{frame}{frm[o]{--}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{--}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldashpat}}
\xP@hook{frame}{frm{,}}
\expandafter\newcommand\expandafter*\csname xP@frm{,}\endcsname{\xP@framedrop\xP@frameshadow
}
\newcommand*\xP@frameshadow[1]{\R@#1\relax
\ifdim\R@=\z@\R@1.2pt\relax\fi
\xP@frameifnotzero\xP@shadow
}
\newcommand*\xP@shadow{\hskip\dimexpr\R@c+\R@/2\relax
\lower\dimexpr\D@c+\R@/2\relax\hbox{\def\xP@pattern{0 J 0 j []0 d}\edef\xP@lw{\xP@dim\R@}\xP@stroke{\xP@dim{\R@/2-\L@c-\R@c} 0 m 0 0 l 0 \xP@dim{\D@c+\U@c-\R@/2}l}}}
\xP@hook{frame}{frm{o-}}
\expandafter\newcommand\expandafter*\csname xP@frm{o-}\endcsname{\xP@framedrop\xP@roundedrectframe
}
\newcommand*\xP@roundedrectframe[1]{\R@#1\relax
\ifdim\R@=\z@\R@\xydashl@\relax\fi
\xP@frameifnotzero\xP@roundedrectangle
}
\newcommand*\xP@roundedrectangle{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\R@\xP@min\R@{.5\dimen@}\R@\xP@min\R@{.5\dimen@ii}\hskip-\L@c
\lower\D@c\hbox{\@tempdimb\dimexpr2\dimen@+2\dimen@ii-\R@*696621973/405764219\relax
\def\@tempa{*119763188/267309217}\xP@setsolidpat
\xP@stroke{\xP@dim\R@0 m \xP@dim{\R@\@tempa}0 0 \xP@dim{\R@\@tempa}0 \xP@dim\R@ c \ifdim2\R@=\dimen@ii\else
0 \xP@dim{\dimen@ii-\R@}m \fi
0 \xP@dim{\dimen@ii-\R@\@tempa}\xP@coor{\R@\@tempa}\dimen@ii
\xP@coor\R@\dimen@ii c \ifdim2\R@=\dimen@\else
\xP@coor{\dimen@-\R@}\dimen@ii m \fi
\xP@coor{\dimen@-\R@\@tempa}\dimen@ii
\xP@coor\dimen@{\dimen@ii-\R@\@tempa}\xP@coor\dimen@{\dimen@ii-\R@} c \ifdim2\R@=\dimen@ii\else
\xP@coor\dimen@\R@ m \fi
\xP@coor\dimen@{\R@\@tempa}\xP@dim{\dimen@-\R@\@tempa}0 \xP@dim{\dimen@-\R@}0 c}\xP@contfalse
\@tempdimb\dimexpr\L@c+\R@c-2\R@\relax
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\xP@setdashpat
\ifdim\@tempdima>\z@
\dimen@\dimexpr\@tempdimb+\R@-\@tempdima/2\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\xP@stroke{\xP@dim{\R@+\@tempdima}0 m \xP@dim\dimen@ 0 l \xP@coor{\R@+\@tempdima}\dimen@ii m \xP@coor\dimen@\dimen@ii l}\fi
\@tempdimb\dimexpr\U@c+\D@c-2\R@\relax
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\xP@setdashpat
\ifdim\@tempdima>\z@
\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\@tempdimb+\R@-\@tempdima/2\relax
\xP@stroke{0 \xP@dim{\R@+\@tempdima}m 0 \xP@dim\dimen@ii l \xP@coor\dimen@{\R@+\@tempdima}m \xP@coor\dimen@\dimen@ii l}\fi
}}
\xP@hook{frame}{frm{=}}
\expandafter\newcommand\expandafter*\csname xP@frm{=}\endcsname{\xP@framedrop\xP@dsframe
}
\newcommand*\xP@dsframe[1]{\R@#1\relax
\xP@frameifnotzero\xP@dsoval
}
\newcommand*\xP@dsoval{\dimen@\dimexpr(\L@c+\R@c)/2\relax
\ifdim\dimen@<\xydashh@\dimen@\xydashh@\fi
\dimen@ii\dimexpr(\U@c+\D@c)/2\relax
\ifdim\dimen@ii<\xydashh@\dimen@ii\xydashh@\fi
\R@\xP@min\R@\dimen@
\R@\xP@min\R@\dimen@ii
\xP@setsolidpat
\let\xP@fillorstroke\xP@stroke
\xP@oval
\hskip\L@c
\advance\L@c-\xydashh@
\advance\R@c-\xydashh@
\advance\U@c-\xydashh@
\advance\D@c-\xydashh@
\advance\R@-\xydashh@
\ifdim\R@<\z@\R@\z@\fi
\xP@oval
}
\xP@hook{frame}{frm[o]{=}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{=}\endcsname{\xP@framedrop\xP@dsellframe
}
\xP@hook{frame}{frm{ee}}
\expandafter\newcommand\expandafter*\csname xP@frm{ee}\endcsname{\xP@framedrop\xP@dsellframe
}
\newcommand*\xP@dsellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsellipse
}
\@ifdefinable\xP@temppath\relax
\newcommand*\xP@dsellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\advance\A@-\xydashh@
\advance\B@-\xydashh@
\ifdim\A@<\z@\A@\z@\fi
\ifdim\B@<\z@\B@\z@\fi
\def\xP@fillorstroke{\edef\xP@temppath}\xP@ellipse@
\xP@inibigdim
\let\@tempa\xydashh@
\xP@offsetellipse
\xP@setsolidpat
\xP@stroke{\xP@temppath\space\the\@temptokena}}}
\newcommand*\xP@offsetellipse{\xP@movetotrue
\@temptokena{}\xP@offsetelliptseg\A@\z@\A@{\B@*173517671/654249180}{\A@*554561898/619869377}{\B@*34221476/65864945}{\A@*543339720/768398401}{\B@*543339720/768398401}\xP@offsetelliptseg{\A@*543339720/768398401}{\B@*543339720/768398401}{\A@*34221476/65864945}{\B@*554561898/619869377}{\A@*173517671/654249180}\B@\z@\B@
\xP@mirrorpath
}
\newcommand*\xP@mirrorpath{\edef\@tempa{\the\@temptokena\relax\space\space\space\space}\let\@tempb\@empty
\let\@tempc\@empty
\expandafter\xP@mirrorpath@\@tempa
}
\@ifdefinable\xP@mirrorpath@\relax
\def\xP@mirrorpath@#1 #2 #3 #4 #5 #6 #7 {\ifx\relax#4\xP@append\@temptokena{\@tempb\xP@minus#1 \xP@minus#2 #3 \@tempc h}\else
\edef\@tempb{\xP@minus#6 #7 \xP@minus#4 #5 \xP@minus#1 #2 c \@tempb\if#3m\else\xP@minus#1 \xP@minus#2 #3 \fi\xP@minus#4 \xP@minus#5 \xP@minus#6 \xP@minus#7 }\edef\@tempc{#6 \xP@minus#7 #4 \xP@minus#5 #1 \xP@minus#2 c \@tempc}\expandafter\xP@mirrorpath@
\fi
}
\@ifdefinable\xP@minus\relax
\def\xP@minus#1 {\if-#1 \else\ifdim\dimexpr#1pt\relax=\z@\else-\fi#1 \fi}
\newcommand*\xP@insertbefore[2]{{\edef\@tempa{#1{#2\the#1}}\expandafter}\@tempa}
\newcommand*\xP@offsetelliptseg[8]{\X@p\dimexpr#1\relax
\Y@p\dimexpr#2\relax
\L@c\dimexpr#3\relax
\U@c\dimexpr#4\relax
\R@c\dimexpr#5\relax
\D@c\dimexpr#6\relax
\X@c\dimexpr#7\relax
\Y@c\dimexpr#8\relax
\xP@savepts
\xP@a\z@
\xP@c\xP@bigdim
\xP@paintsolid@
}
\newcommand*\xP@getradii[1]{\edef\@tempa{#1}\expandafter\xP@getradii@\@tempa,\maxdimen,@}
\@ifdefinable\xP@getradii@\relax
\def\xP@getradii@#1,#2,#3@{\A@#1\relax
\B@#2\relax
\ifdim\B@=\maxdimen
\A@\dimexpr(\L@c+\R@c)/2\relax
\B@\dimexpr(\U@c+\D@c)/2\relax
\fi
}
\xP@hook{frame}{frm{o}}
\expandafter\newcommand\expandafter*\csname xP@frm{o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setsolidpat}}
\xP@hook{frame}{frm{-o}}
\expandafter\newcommand\expandafter*\csname xP@frm{-o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setcldashpat}}
\xP@hook{frame}{frm{.o}}
\expandafter\newcommand\expandafter*\csname xP@frm{.o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setcldottedpat}}
\newcommand*\xP@circleframe[2]{\R@#2\relax
\def\xP@fillorstroke{#1\xP@stroke}\DN@{\zeroEdge}\ifx\next@\prevEdge@@
\ifdim\R@>\z@
\xP@circleframe@
\fi
\else
\ifdim\R@=\z@
\A@\dimexpr(\L@c+\R@c)/2\relax
\B@\dimexpr(\U@c+\D@c)/2\relax
\R@\xP@max\A@\B@
\fi
\xP@circleframe@
\fi
}
\newcommand*\xP@circleframe@{\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\xP@circle}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\xP@hook{frame}{frm{e}}
\expandafter\newcommand\expandafter*\csname xP@frm{e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setsolidpat}}
\xP@hook{frame}{frm{-e}}
\expandafter\newcommand\expandafter*\csname xP@frm{-e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldashpat}}
\xP@hook{frame}{frm{.e}}
\expandafter\newcommand\expandafter*\csname xP@frm{.e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldottedpat}}
\xP@hook{frame}{frm2{.e}}
\expandafter\newcommand\expandafter*\csname xP@frm2{.e}\endcsname{\xP@framedrop\xP@dsdottedellframe
}
\newcommand*\xP@dsdottedellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsdottedellipse
}
\newcommand*\xP@dsdottedellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\@tempdima.5\xydashh@\relax
\advance\A@-\@tempdima
\advance\B@-\@tempdima
\ifdim\A@<\@tempdima\A@\@tempdima\fi
\ifdim\B@<\@tempdima\B@\@tempdima\fi
\let\xP@normalmult\@ne
\xP@specialellipse{\xP@splinemultdotted\xP@doublestroke}}}
\newcommand*\xP@specialellipse[1]{\def\@tempa{*147546029/267309217}\X@p\A@
\Y@p\z@
\L@c\A@
\U@c\dimexpr\B@\@tempa\relax
\R@c\dimexpr\A@\@tempa\relax
\D@c\B@
\X@c\z@
\Y@c\B@
\xP@bezierlength
\let\xP@testcont\xP@alwaysconttrue
#1\X@p\z@
\Y@p\B@
\L@c-\R@c
\D@c\U@c
\U@c\B@
\R@c-\A@
\X@c-\A@
\Y@c\z@
#1\X@p-\A@
\Y@p\z@
\R@c\L@c
\L@c-\A@
\U@c-\D@c
\D@c-\B@
\X@c\z@
\Y@c-\B@
#1\X@p\z@
\Y@p-\B@
\L@c-\R@c
\D@c\U@c
\U@c-\B@
\R@c\A@
\X@c\A@
\Y@c\z@
#1}
\newcommand*\xP@alwaysconttrue[1]{\xP@splineconttrue}
\xP@hook{frame}{frm2{-e}}
\expandafter\newcommand\expandafter*\csname xP@frm2{-e}\endcsname{\xP@framedrop\xP@dsdashellframe
}
\newcommand*\xP@dsdashellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsdashellipse
}
\newcommand*\xP@dsdashellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\advance\A@-\xydashh@
\advance\B@-\xydashh@
\ifdim\A@<\z@\A@\z@\fi
\ifdim\B@<\z@\B@\z@\fi
\xP@specialellipse{\xP@splinemultdashed\xP@elldoublestroke}}}
\newcommand*\xP@elldoublestroke{\z@,\xydashh@}
\newcommand*\xP@fill[1]{\xP@literal{#1 f}}
\newcommand*\xP@fillstroke[1]{\xP@literal{\xP@dim{\xP@preclw/2}w 1 j 0 G #1 b}}
\newcommand*\xP@fillorstroke{}
\xP@hook{frame}{frm{*}}
\expandafter\newcommand\expandafter*\csname xP@frm{*}\endcsname{\xP@framedrop{\let\xP@fillorstroke\xP@fill\xP@framefill}}
\xP@hook{frame}{frm{**}}
\expandafter\newcommand\expandafter*\csname xP@frm{**}\endcsname{\xP@framedrop{\let\xP@fillorstroke\xP@fillstroke\xP@framefill}}
\newcommand*\xP@framefill[1]{\R@#1\relax
\xP@setsolidpat
\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\DN@{\rectangleEdge}\ifx\next@\prevEdge@@
\DN@{\xP@oval}\else
\DN@{\circleEdge}\ifx\next@\prevEdge@@
\ifdim\R@=\z@
\DN@{\xP@filledellipse}\else
\DN@{\restR@max\xP@circle}\fi
\else
\ifdim\R@=\z@
\DN@{\xP@oval}\else
\DN@{\xP@circle}\fi
\fi
\fi
\next@
}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\newcommand*\xP@circle{\xP@ellipse\R@\R@
}
\newcommand*\xP@filledellipse{\xP@ellipse{\dimexpr(\L@c+\R@c)/2\relax}{\dimexpr(\U@c+\D@c)/2\relax}}
\newcommand*\xP@framedellipse{\xP@ellipse\A@\B@
}
\newcommand*\xP@ellipse[2]{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\A@#1\relax
\B@#2\relax
\xP@ellipse@
}}
\newcommand*\xP@ellipse@{\X@p\dimexpr\A@*543339720/768398401\relax
\Y@p\dimexpr\B@*543339720/768398401\relax
\L@c\dimexpr\A@*34221476/65864945\relax
\U@c\dimexpr\B@*554561898/619869377\relax
\R@c\dimexpr\A@*173517671/654249180\relax
\D@c\B@
\X@c\z@
\Y@c\B@
\xP@bezierlength
\@tempdima\@tempdimb
\X@p\A@
\Y@p\z@
\L@c\A@
\U@c\dimexpr\B@*173517671/654249180\relax
\R@c\dimexpr\A@*554561898/619869377\relax
\D@c\dimexpr\B@*34221476/65864945\relax
\X@c\dimexpr\A@*543339720/768398401\relax
\Y@c\dimexpr\B@*543339720/768398401\relax
\xP@bezierlength
\@tempdimb4\dimexpr\@tempdima+\@tempdimb\relax
\edef\@tempa{\xP@dim\A@0 m
\xP@coor\L@c\U@c
\xP@coor\R@c\D@c
\xP@coor\X@c\Y@c c \xP@coor{\A@*34221476/65864945}{\B@*554561898/619869377}\xP@coor{\A@*173517671/654249180}\B@
0 \xP@dim\B@ c }\@temptokena\expandafter{\@tempa}\xP@mirrorpath
\xP@fillorstroke{\the\@temptokena}}
\xyendinput
%%
%% End of file `xypdf-fr.tex'.


==> xypdf-li.tex <==
%auto-ignore
%%
%% This is file `xypdf-fr.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `frame')
%%
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://www.math.uni-bonn.de/people/muellner>
%% --------------------------------------------------------------------------
%%
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%%
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%%
%% --------------------------------------------------------------------------
%%
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%%
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%%
%% The files with the TeX code are generated by the following command:
%%
%%    latex xypdf.ins
%%
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%%
%% --------------------------------------------------------------------------
%%
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%%
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%%

\xyrequire{curve}\xycatcodes
\expandafter\let\csname xypdf-fr@loaded\endcsname\@empty
\newcommand*\xP@framedrop[1]{\expandafter\frmDrop@\expandafter{\expandafter\def\expandafter\prevEdge@@\expandafter{\prevEdge@@}#1\frmradius@@}}
\xP@hook{frame}{frm{-}}
\expandafter\newcommand\expandafter*\csname xP@frm{-}\endcsname{\xP@framedrop\xP@solidframe
}
\newcommand*\xP@solidframe[1]{\R@#1\relax
\xP@setsolidpat
\let\xP@fillorstroke\xP@stroke
\xP@frameifnotzero\xP@oval
}
\newcommand*\xP@frameifnotzero[1]{\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\DN@{\zeroEdge}\ifx\next@\prevEdge@@
\else
#1\fi
}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\newcommand*\xP@oval{\hskip-\L@c
\lower\D@c\hbox{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\R@\xP@min\R@{.5\dimen@}\R@\xP@min\R@{.5\dimen@ii}\@tempdimb\dimexpr2\dimen@+2\dimen@ii-\R@*696621973/405764219\relax
\ifdim\R@=\z@
\xP@fillorstroke{0 0 \xP@coor\dimen@\dimen@ii re}\else
\def\@tempa{*119763188/267309217}\xP@fillorstroke{\xP@dim\R@0 m \xP@dim{\R@\@tempa}0 0 \xP@dim{\R@\@tempa}0 \xP@dim\R@ c \ifdim2\R@=\dimen@ii\else
0 \xP@dim{\dimen@ii-\R@}l \fi
0 \xP@dim{\dimen@ii-\R@\@tempa}\xP@coor{\R@\@tempa}\dimen@ii
\xP@coor\R@\dimen@ii c \ifdim2\R@=\dimen@\else
\xP@coor{\dimen@-\R@}\dimen@ii l \fi
\xP@coor{\dimen@-\R@\@tempa}\dimen@ii
\xP@coor\dimen@{\dimen@ii-\R@\@tempa}\xP@coor\dimen@{\dimen@ii-\R@} c \ifdim2\R@=\dimen@ii\else
\xP@coor\dimen@\R@ l \fi
\xP@coor\dimen@{\R@\@tempa}\xP@dim{\dimen@-\R@\@tempa}0 \xP@dim{\dimen@-\R@}0 c h}\fi
}}
\xP@hook{frame}{frm[o]{-}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{-}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setsolidpat}}
\newcommand*\xP@ellipseframe[2]{\xP@getradii{#2}\DN@{\zeroEdge}\ifx\next@\prevEdge@@
\else
\def\xP@fillorstroke{#1\xP@stroke}\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\xP@framedellipse}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
\fi
}
\xP@hook{frame}{frm{.}}
\expandafter\newcommand\expandafter*\csname xP@frm{.}\endcsname{\xP@framedrop\xP@rectframedotted
}
\newcommand*\xP@rectframedotted[1]{\R@#1\relax
\xP@frameifnotzero{\ifdim\R@=\z@
\xP@dottedrect
\else
\xP@dottedoval
\fi
}}
\newcommand*\xP@dottedrect{\hskip-\L@c
\lower\D@c\hbox{\dimen@ii\dimexpr\U@c+\D@c\relax
\@tempdimc\dimexpr\xP@preclw/-2\relax
\@tempdimb\dimexpr\L@c+\R@c+\xP@preclw\relax
\xP@contfalse
\xP@setdottedpat
\dimen@\dimexpr\@tempdimb+\@tempdima/2+\@tempdimc\relax
\xP@stroke{\xP@dim\@tempdimc0 m \xP@dim\dimen@0 l \xP@coor\@tempdimc\dimen@ii m \xP@coor\dimen@\dimen@ii l}\let\xP@testcont\xP@alwaysconttrue
\@tempdimb\dimen@ii
\xP@setdottedpat
\dimen@\dimexpr\L@c+\R@c\relax
\advance\dimen@ii\dimexpr\@tempdimc-\@tempdima/2\relax
\multiply\@tempdimc\m@ne
\xP@stroke{0 \xP@dim\@tempdimc m 0 \xP@dim\dimen@ii l \xP@coor\dimen@\@tempdimc m \xP@coor\dimen@\dimen@ii l}}}
\newcommand*\xP@dottedoval{\def\xP@fillorstroke{\xP@setcldottedpat\xP@stroke}\xP@oval
}
\xP@hook{frame}{frm[o]{.}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{.}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldottedpat}}
\xP@hook{frame}{frm{--}}
\expandafter\newcommand\expandafter*\csname xP@frm{--}\endcsname{\xP@framedrop\xP@rectframedashed
}
\newcommand*\xP@rectframedashed[1]{\R@#1\relax
\xP@frameifnotzero{\ifdim\R@=\z@
\xP@dashedrect
\else
\xP@dashedoval
\fi
}}
\newcommand*\xP@dashedrect{\hskip-\L@c
\lower\D@c\hbox{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\@tempdimb\dimen@
\xP@contfalse
\xP@setdashpat
\xP@stroke{0 0 m \xP@dim\dimen@0 l 0 \xP@dim\dimen@ii m \xP@coor\dimen@\dimen@ii l}\@tempdimb\dimen@ii
\xP@setdashpat
\xP@stroke{0 0 m 0 \xP@dim\dimen@ii l \xP@dim\dimen@0 m \xP@coor\dimen@\dimen@ii l}}}
\newcommand*\xP@dashedoval{\def\xP@fillorstroke{\xP@setcldashpat\xP@stroke}\xP@oval
}
\xP@hook{frame}{frm[o]{--}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{--}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldashpat}}
\xP@hook{frame}{frm{,}}
\expandafter\newcommand\expandafter*\csname xP@frm{,}\endcsname{\xP@framedrop\xP@frameshadow
}
\newcommand*\xP@frameshadow[1]{\R@#1\relax
\ifdim\R@=\z@\R@1.2pt\relax\fi
\xP@frameifnotzero\xP@shadow
}
\newcommand*\xP@shadow{\hskip\dimexpr\R@c+\R@/2\relax
\lower\dimexpr\D@c+\R@/2\relax\hbox{\def\xP@pattern{0 J 0 j []0 d}\edef\xP@lw{\xP@dim\R@}\xP@stroke{\xP@dim{\R@/2-\L@c-\R@c} 0 m 0 0 l 0 \xP@dim{\D@c+\U@c-\R@/2}l}}}
\xP@hook{frame}{frm{o-}}
\expandafter\newcommand\expandafter*\csname xP@frm{o-}\endcsname{\xP@framedrop\xP@roundedrectframe
}
\newcommand*\xP@roundedrectframe[1]{\R@#1\relax
\ifdim\R@=\z@\R@\xydashl@\relax\fi
\xP@frameifnotzero\xP@roundedrectangle
}
\newcommand*\xP@roundedrectangle{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\R@\xP@min\R@{.5\dimen@}\R@\xP@min\R@{.5\dimen@ii}\hskip-\L@c
\lower\D@c\hbox{\@tempdimb\dimexpr2\dimen@+2\dimen@ii-\R@*696621973/405764219\relax
\def\@tempa{*119763188/267309217}\xP@setsolidpat
\xP@stroke{\xP@dim\R@0 m \xP@dim{\R@\@tempa}0 0 \xP@dim{\R@\@tempa}0 \xP@dim\R@ c \ifdim2\R@=\dimen@ii\else
0 \xP@dim{\dimen@ii-\R@}m \fi
0 \xP@dim{\dimen@ii-\R@\@tempa}\xP@coor{\R@\@tempa}\dimen@ii
\xP@coor\R@\dimen@ii c \ifdim2\R@=\dimen@\else
\xP@coor{\dimen@-\R@}\dimen@ii m \fi
\xP@coor{\dimen@-\R@\@tempa}\dimen@ii
\xP@coor\dimen@{\dimen@ii-\R@\@tempa}\xP@coor\dimen@{\dimen@ii-\R@} c \ifdim2\R@=\dimen@ii\else
\xP@coor\dimen@\R@ m \fi
\xP@coor\dimen@{\R@\@tempa}\xP@dim{\dimen@-\R@\@tempa}0 \xP@dim{\dimen@-\R@}0 c}\xP@contfalse
\@tempdimb\dimexpr\L@c+\R@c-2\R@\relax
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\xP@setdashpat
\ifdim\@tempdima>\z@
\dimen@\dimexpr\@tempdimb+\R@-\@tempdima/2\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\xP@stroke{\xP@dim{\R@+\@tempdima}0 m \xP@dim\dimen@ 0 l \xP@coor{\R@+\@tempdima}\dimen@ii m \xP@coor\dimen@\dimen@ii l}\fi
\@tempdimb\dimexpr\U@c+\D@c-2\R@\relax
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\xP@setdashpat
\ifdim\@tempdima>\z@
\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\@tempdimb+\R@-\@tempdima/2\relax
\xP@stroke{0 \xP@dim{\R@+\@tempdima}m 0 \xP@dim\dimen@ii l \xP@coor\dimen@{\R@+\@tempdima}m \xP@coor\dimen@\dimen@ii l}\fi
}}
\xP@hook{frame}{frm{=}}
\expandafter\newcommand\expandafter*\csname xP@frm{=}\endcsname{\xP@framedrop\xP@dsframe
}
\newcommand*\xP@dsframe[1]{\R@#1\relax
\xP@frameifnotzero\xP@dsoval
}
\newcommand*\xP@dsoval{\dimen@\dimexpr(\L@c+\R@c)/2\relax
\ifdim\dimen@<\xydashh@\dimen@\xydashh@\fi
\dimen@ii\dimexpr(\U@c+\D@c)/2\relax
\ifdim\dimen@ii<\xydashh@\dimen@ii\xydashh@\fi
\R@\xP@min\R@\dimen@
\R@\xP@min\R@\dimen@ii
\xP@setsolidpat
\let\xP@fillorstroke\xP@stroke
\xP@oval
\hskip\L@c
\advance\L@c-\xydashh@
\advance\R@c-\xydashh@
\advance\U@c-\xydashh@
\advance\D@c-\xydashh@
\advance\R@-\xydashh@
\ifdim\R@<\z@\R@\z@\fi
\xP@oval
}
\xP@hook{frame}{frm[o]{=}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{=}\endcsname{\xP@framedrop\xP@dsellframe
}
\xP@hook{frame}{frm{ee}}
\expandafter\newcommand\expandafter*\csname xP@frm{ee}\endcsname{\xP@framedrop\xP@dsellframe
}
\newcommand*\xP@dsellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsellipse
}
\@ifdefinable\xP@temppath\relax
\newcommand*\xP@dsellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\advance\A@-\xydashh@
\advance\B@-\xydashh@
\ifdim\A@<\z@\A@\z@\fi
\ifdim\B@<\z@\B@\z@\fi
\def\xP@fillorstroke{\edef\xP@temppath}\xP@ellipse@
\xP@inibigdim
\let\@tempa\xydashh@
\xP@offsetellipse
\xP@setsolidpat
\xP@stroke{\xP@temppath\space\the\@temptokena}}}
\newcommand*\xP@offsetellipse{\xP@movetotrue
\@temptokena{}\xP@offsetelliptseg\A@\z@\A@{\B@*173517671/654249180}{\A@*554561898/619869377}{\B@*34221476/65864945}{\A@*543339720/768398401}{\B@*543339720/768398401}\xP@offsetelliptseg{\A@*543339720/768398401}{\B@*543339720/768398401}{\A@*34221476/65864945}{\B@*554561898/619869377}{\A@*173517671/654249180}\B@\z@\B@
\xP@mirrorpath
}
\newcommand*\xP@mirrorpath{\edef\@tempa{\the\@temptokena\relax\space\space\space\space}\let\@tempb\@empty
\let\@tempc\@empty
\expandafter\xP@mirrorpath@\@tempa
}
\@ifdefinable\xP@mirrorpath@\relax
\def\xP@mirrorpath@#1 #2 #3 #4 #5 #6 #7 {\ifx\relax#4\xP@append\@temptokena{\@tempb\xP@minus#1 \xP@minus#2 #3 \@tempc h}\else
\edef\@tempb{\xP@minus#6 #7 \xP@minus#4 #5 \xP@minus#1 #2 c \@tempb\if#3m\else\xP@minus#1 \xP@minus#2 #3 \fi\xP@minus#4 \xP@minus#5 \xP@minus#6 \xP@minus#7 }\edef\@tempc{#6 \xP@minus#7 #4 \xP@minus#5 #1 \xP@minus#2 c \@tempc}\expandafter\xP@mirrorpath@
\fi
}
\@ifdefinable\xP@minus\relax
\def\xP@minus#1 {\if-#1 \else\ifdim\dimexpr#1pt\relax=\z@\else-\fi#1 \fi}
\newcommand*\xP@insertbefore[2]{{\edef\@tempa{#1{#2\the#1}}\expandafter}\@tempa}
\newcommand*\xP@offsetelliptseg[8]{\X@p\dimexpr#1\relax
\Y@p\dimexpr#2\relax
\L@c\dimexpr#3\relax
\U@c\dimexpr#4\relax
\R@c\dimexpr#5\relax
\D@c\dimexpr#6\relax
\X@c\dimexpr#7\relax
\Y@c\dimexpr#8\relax
\xP@savepts
\xP@a\z@
\xP@c\xP@bigdim
\xP@paintsolid@
}
\newcommand*\xP@getradii[1]{\edef\@tempa{#1}\expandafter\xP@getradii@\@tempa,\maxdimen,@}
\@ifdefinable\xP@getradii@\relax
\def\xP@getradii@#1,#2,#3@{\A@#1\relax
\B@#2\relax
\ifdim\B@=\maxdimen
\A@\dimexpr(\L@c+\R@c)/2\relax
\B@\dimexpr(\U@c+\D@c)/2\relax
\fi
}
\xP@hook{frame}{frm{o}}
\expandafter\newcommand\expandafter*\csname xP@frm{o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setsolidpat}}
\xP@hook{frame}{frm{-o}}
\expandafter\newcommand\expandafter*\csname xP@frm{-o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setcldashpat}}
\xP@hook{frame}{frm{.o}}
\expandafter\newcommand\expandafter*\csname xP@frm{.o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setcldottedpat}}
\newcommand*\xP@circleframe[2]{\R@#2\relax
\def\xP@fillorstroke{#1\xP@stroke}\DN@{\zeroEdge}\ifx\next@\prevEdge@@
\ifdim\R@>\z@
\xP@circleframe@
\fi
\else
\ifdim\R@=\z@
\A@\dimexpr(\L@c+\R@c)/2\relax
\B@\dimexpr(\U@c+\D@c)/2\relax
\R@\xP@max\A@\B@
\fi
\xP@circleframe@
\fi
}
\newcommand*\xP@circleframe@{\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\xP@circle}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\xP@hook{frame}{frm{e}}
\expandafter\newcommand\expandafter*\csname xP@frm{e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setsolidpat}}
\xP@hook{frame}{frm{-e}}
\expandafter\newcommand\expandafter*\csname xP@frm{-e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldashpat}}
\xP@hook{frame}{frm{.e}}
\expandafter\newcommand\expandafter*\csname xP@frm{.e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldottedpat}}
\xP@hook{frame}{frm2{.e}}
\expandafter\newcommand\expandafter*\csname xP@frm2{.e}\endcsname{\xP@framedrop\xP@dsdottedellframe
}
\newcommand*\xP@dsdottedellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsdottedellipse
}
\newcommand*\xP@dsdottedellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\@tempdima.5\xydashh@\relax
\advance\A@-\@tempdima
\advance\B@-\@tempdima
\ifdim\A@<\@tempdima\A@\@tempdima\fi
\ifdim\B@<\@tempdima\B@\@tempdima\fi
\let\xP@normalmult\@ne
\xP@specialellipse{\xP@splinemultdotted\xP@doublestroke}}}
\newcommand*\xP@specialellipse[1]{\def\@tempa{*147546029/267309217}\X@p\A@
\Y@p\z@
\L@c\A@
\U@c\dimexpr\B@\@tempa\relax
\R@c\dimexpr\A@\@tempa\relax
\D@c\B@
\X@c\z@
\Y@c\B@
\xP@bezierlength
\let\xP@testcont\xP@alwaysconttrue
#1\X@p\z@
\Y@p\B@
\L@c-\R@c
\D@c\U@c
\U@c\B@
\R@c-\A@
\X@c-\A@
\Y@c\z@
#1\X@p-\A@
\Y@p\z@
\R@c\L@c
\L@c-\A@
\U@c-\D@c
\D@c-\B@
\X@c\z@
\Y@c-\B@
#1\X@p\z@
\Y@p-\B@
\L@c-\R@c
\D@c\U@c
\U@c-\B@
\R@c\A@
\X@c\A@
\Y@c\z@
#1}
\newcommand*\xP@alwaysconttrue[1]{\xP@splineconttrue}
\xP@hook{frame}{frm2{-e}}
\expandafter\newcommand\expandafter*\csname xP@frm2{-e}\endcsname{\xP@framedrop\xP@dsdashellframe
}
\newcommand*\xP@dsdashellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsdashellipse
}
\newcommand*\xP@dsdashellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\advance\A@-\xydashh@
\advance\B@-\xydashh@
\ifdim\A@<\z@\A@\z@\fi
\ifdim\B@<\z@\B@\z@\fi
\xP@specialellipse{\xP@splinemultdashed\xP@elldoublestroke}}}
\newcommand*\xP@elldoublestroke{\z@,\xydashh@}
\newcommand*\xP@fill[1]{\xP@literal{#1 f}}
\newcommand*\xP@fillstroke[1]{\xP@literal{\xP@dim{\xP@preclw/2}w 1 j 0 G #1 b}}
\newcommand*\xP@fillorstroke{}
\xP@hook{frame}{frm{*}}
\expandafter\newcommand\expandafter*\csname xP@frm{*}\endcsname{\xP@framedrop{\let\xP@fillorstroke\xP@fill\xP@framefill}}
\xP@hook{frame}{frm{**}}
\expandafter\newcommand\expandafter*\csname xP@frm{**}\endcsname{\xP@framedrop{\let\xP@fillorstroke\xP@fillstroke\xP@framefill}}
\newcommand*\xP@framefill[1]{\R@#1\relax
\xP@setsolidpat
\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\DN@{\rectangleEdge}\ifx\next@\prevEdge@@
\DN@{\xP@oval}\else
\DN@{\circleEdge}\ifx\next@\prevEdge@@
\ifdim\R@=\z@
\DN@{\xP@filledellipse}\else
\DN@{\restR@max\xP@circle}\fi
\else
\ifdim\R@=\z@
\DN@{\xP@oval}\else
\DN@{\xP@circle}\fi
\fi
\fi
\next@
}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\newcommand*\xP@circle{\xP@ellipse\R@\R@
}
\newcommand*\xP@filledellipse{\xP@ellipse{\dimexpr(\L@c+\R@c)/2\relax}{\dimexpr(\U@c+\D@c)/2\relax}}
\newcommand*\xP@framedellipse{\xP@ellipse\A@\B@
}
\newcommand*\xP@ellipse[2]{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\A@#1\relax
\B@#2\relax
\xP@ellipse@
}}
\newcommand*\xP@ellipse@{\X@p\dimexpr\A@*543339720/768398401\relax
\Y@p\dimexpr\B@*543339720/768398401\relax
\L@c\dimexpr\A@*34221476/65864945\relax
\U@c\dimexpr\B@*554561898/619869377\relax
\R@c\dimexpr\A@*173517671/654249180\relax
\D@c\B@
\X@c\z@
\Y@c\B@
\xP@bezierlength
\@tempdima\@tempdimb
\X@p\A@
\Y@p\z@
\L@c\A@
\U@c\dimexpr\B@*173517671/654249180\relax
\R@c\dimexpr\A@*554561898/619869377\relax
\D@c\dimexpr\B@*34221476/65864945\relax
\X@c\dimexpr\A@*543339720/768398401\relax
\Y@c\dimexpr\B@*543339720/768398401\relax
\xP@bezierlength
\@tempdimb4\dimexpr\@tempdima+\@tempdimb\relax
\edef\@tempa{\xP@dim\A@0 m
\xP@coor\L@c\U@c
\xP@coor\R@c\D@c
\xP@coor\X@c\Y@c c \xP@coor{\A@*34221476/65864945}{\B@*554561898/619869377}\xP@coor{\A@*173517671/654249180}\B@
0 \xP@dim\B@ c }\@temptokena\expandafter{\@tempa}\xP@mirrorpath
\xP@fillorstroke{\the\@temptokena}}
\xyendinput
%%
%% End of file `xypdf-fr.tex'.


==> xypdf-ro.tex <==
%auto-ignore
%%
%% This is file `xypdf-ro.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `rotate')
%%
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://www.math.uni-bonn.de/people/muellner>
%% --------------------------------------------------------------------------
%%
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%%
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%%
%% --------------------------------------------------------------------------
%%
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%%
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%%
%% The files with the TeX code are generated by the following command:
%%
%%    latex xypdf.ins
%%
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%%
%% --------------------------------------------------------------------------
%%
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%%
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%%

\xycatcodes
\expandafter\let\csname xypdf-ro@loaded\endcsname\@empty
\xP@hook{rotate}{xyscale@@}
\newcommand*\xP@xyscale@@[2]{\setboxz@h{\hskip\L@p
\hskip-\R@p
\lower\U@p\hbox{\xP@cm{#1}00{#2}{\raise\U@p\hb@xt@\z@{\hskip-\L@p\boxz@\hss}}}}\global\let\xP@lastpattern\@empty
}
\xP@hook{rotate}{xyRotate@@}
\newcommand\xP@xyRotate@@{\xP@rotate@\xP@trigfromdir}
\xP@hook{rotate}{doSpecialRotate@@}
\@ifdefinable\xP@doSpecialRotate@@\relax
\def\xP@doSpecialRotate@@#1@@{\xP@rotate@\xP@trig{#1}}
\newcommand*\xP@rotate@[2]{\setboxz@h{#1{#2}\hskip\L@p
\hskip-\R@p
\lower\U@p\hbox{\xP@cm\cosDirection\sinDirection
{\if-\sinDirection\else-\sinDirection\fi}\cosDirection
{\raise\U@p\hb@xt@\z@{\hskip-\L@p\boxz@\hss}}}}\global\let\xP@lastpattern\@empty
}
\newcommand*\xP@trig[1]{\@tempdima\dimexpr#1pt\relax
\@tempdimb\@tempdima
\divide\@tempdimb23592960
\advance\@tempdima-23592960\@tempdimb
\ifdim\@tempdima<\z@\advance\@tempdima360pt\fi
\@tempdimb\@tempdima
\divide\@tempdimb5898240
\ifcase\@tempdimb
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\@tempdimb}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\@tempdimb}\or
\@tempdima\dimexpr180pt-\@tempdima\relax
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\@tempdimb}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\or
\@tempdima\dimexpr\@tempdima-180pt\relax
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\or
\@tempdima\dimexpr360pt-\@tempdima\relax
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\@tempdimb}\else
\PackageError{xypdf}{Unexpected case in sin/cos calculation}{Feel free to contact the author of the xypdf package with a minimal example.}\fi
}
\newcommand*\xP@sinpoly{{\ifdim\@tempdima<49pt
\ifdim\@tempdima<27pt
\@tempdimb\dimexpr((\@tempdima*-529771058/16039085-1384933sp)*\@tempdima/268756075+10714164sp)*\@tempdima/613777813\relax
\else
\advance\@tempdima-27pt
\@tempdimb\dimexpr(((\@tempdima*-743101305/20672414-238989613sp)*\@tempdima/80975565+42661556sp)*\@tempdima/622461739+2\p@)*157520747/693945047\relax
\fi
\else
\ifdim\@tempdima<70pt
\advance\@tempdima-49pt
\@tempdimb\dimexpr(((\@tempdima*-348406699/107952940-55079229sp)*\@tempdima/866635628+408805sp)*\@tempdima/26926757+\p@)*135751711/179873976\relax
\else
\advance\@tempdima-70pt
\@tempdimb\dimexpr(((\@tempdima*-1015850353/137849442-460519207sp)*\@tempdima/8742349+142263941sp)*\@tempdima/972432199+23\p@)*31253604/764969669\relax
\fi
\fi
\global\dimen@i\@tempdimb
}\@tempdimb\dimen@i
}
\xyendinput
%%
%% End of file `xypdf-ro.tex'.


==> xypdf.tex <==
%auto-ignore
%%
%% This is file `xypdf.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `basic')
%%
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://www.math.uni-bonn.de/people/muellner>
%% --------------------------------------------------------------------------
%%
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%%
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%%
%% --------------------------------------------------------------------------
%%
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%%
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%%
%% The files with the TeX code are generated by the following command:
%%
%%    latex xypdf.ins
%%
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%%
%% --------------------------------------------------------------------------
%%
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%%
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%%

\ifx\xyloaded\undefined\input xy \fi
\xyprovide{pdf}{PDF driver}{1.5}{Daniel M\"ullner\newline}{\url{http://www.math.uni-bonn.de/people/muellner}}{}
\ifx\makeatletter\undefined\input miniltx \fi
\newcommand*\xypdfdate{2010/10/11}
\newdriver{\xyaddsupport{pdf}\xP@pdf@on
\xyaddsupport{color}\xP@color@on
\xyaddsupport{curve}\xP@curve@on
\xyaddsupport{frame}\xP@frame@on
\xyaddsupport{rotate}\xP@rotate@on
}
\xyaddunsupport{pdf}\xP@pdf@off
\xyaddunsupport{color}\xP@color@off
\xyaddunsupport{curve}\xP@curve@off
\xyaddunsupport{frame}\xP@frame@off
\xyaddunsupport{rotate}\xP@rotate@off
\newcommand*\xypdfon{\xP@pdf@on
\xP@color@on
\xP@curve@on
\xP@frame@on
\xP@line@on
\xP@rotate@on
}
\newcommand*\xypdfoff{\xP@pdf@off
\xP@color@off
\xP@curve@off
\xP@frame@off
\xP@line@off
\xP@rotate@off
}
\ifx\unexpanded\@undefined
\PackageError{xypdf}{eTeX is needed for the xypdf package}{}
\fi
\newcommand*\xP@testpdfsave{\ifpdf
\ifx\pdfsave\@undefined
\PackageError{xypdf}{pdfTeX version 1.40.0 or higher is needed for the xypdf^^Jpackage with PDF output}{}\fi
\fi
\let\xP@testpdfsave\@undefined
}
\ifx\PackageWarning\@undefined
\newcommand*\xP@warning[2]{{\newlinechar`\^^J\@warning{Package #1 Warning: #2\@empty.}}}
\else
\newcommand*\xP@warning{\PackageWarning}
\fi
\newcommand*\xP@pdf@on{}
\newcommand*\xP@pdf@off{}
\newcommand*\xP@color@on{}
\newcommand*\xP@color@off{}
\newcommand*\xP@curve@on{}
\newcommand*\xP@curve@off{}
\newcommand*\xP@frame@on{}
\newcommand*\xP@frame@off{}
\newcommand*\xP@line@on{}
\newcommand*\xP@line@off{}
\newcommand*\xP@rotate@on{}
\newcommand*\xP@rotate@off{}
\newcommand*\xP@hook[2]{\edef\next@{\let\expandafter\noexpand\csname xP@old@#2\endcsname
\expandafter\noexpand\csname#2\endcsname}\next@
\expandafter\edef\csname xP@#1@on\endcsname{\unexpanded\expandafter\expandafter\expandafter{\csname xP@#1@on\endcsname}\let\expandafter\noexpand\csname#2\endcsname
\expandafter\noexpand\csname xP@#2\endcsname
}\expandafter\edef\csname xP@#1@off\endcsname{\unexpanded\expandafter\expandafter\expandafter{\csname xP@#1@off\endcsname}\let\expandafter\noexpand\csname#2\endcsname
\expandafter\noexpand\csname xP@old@#2\endcsname
}}
\newcommand*\xP@defpdfliteral{\ifpdf
\newcommand*\xP@literal[1]{\pdfsave\pdfliteral{##1}\pdfrestore}
\newcommand*\xP@cm[5]{\pdfsave
\pdfsetmatrix{##1 ##2 ##3 ##4}##5\pdfrestore
}
\@ifundefined{@pdfcolorstack}{\def\@pdfcolorstack{\z@}}{}\newcommand*\xP@setcolor[3]{\pdfcolorstack\@pdfcolorstack push{##1 ##2 ##1 ##3}}
\newcommand*\xP@resetcolor{\pdfcolorstack\@pdfcolorstack pop\relax}\else
\newcommand*\xP@literal{\xP@warning{xypdf}{The produced DVI file is NOT PORTABLE. Convert it with^^Jdvipdfm(x) to the PDF format but do not expect the DVI file itself to be^^Jdisplayed correctly\@gobble}\global\let\xP@literal\xP@literal@
\xP@literal
}
\newcommand*\xP@literal@[1]{\special{pdf:content ##1}}
\newcommand*\xP@cm[5]{\special{pdf:btrans matrix ##1 ##2 ##3 ##4 0 0}##5\special{pdf:etrans}}
\newcommand*\xP@setcolor[3]{\special{pdf:bcolor[##1]}}
\newcommand*\xP@resetcolor{\special{pdf:ecolor}}\fi
\let\xP@defpdfliteral\@undefined
}
\DN@{\@firstofone}
\DNii@{xy}
\ifx\@currname\nextii@
\ifx\AtEndOfPackage\@undefined
\else
\DN@{\AtEndOfPackage}\fi
\fi
\next@
{\RequirePackage{ifpdf}\xP@testpdfsave
\xP@defpdfliteral}
\ifx\pdfdecimaldigits\@undefined
\newcommand*\xP@digits{2}
\else
\@ifdefinable\xP@digits\relax
\xdef\xP@digits{\the\pdfdecimaldigits}
\ifnum\pdfdecimaldigits<2
\xP@warning{xypdf}{The precision in \string\pdfdecimaldigits\space is only \xP@digits\space
decimals.^^JIt is recommended to set \string\pdfdecimaldigits\space to 2 or 3 for best output quality\@gobble}
\fi
\fi
\newcommand*\xP@dim[1]{\expandafter\xP@removePT\the\dimexpr(#1)*800/803\relax\space}
\newcommand*\xP@precdim[1]{\xP@EARPT\dimexpr(#1)*800/803\relax\space}
\newcommand*\xP@EARPT{\expandafter\removePT@\the}
\newcommand*\xP@coor[1]{\xP@dim{#1}\xP@dim}
\@ifdefinable\xP@removePT\relax
{\@makeother\p\@makeother\t\gdef\xP@removePT#1pt{\xP@removePT@#10000@}}
\@ifdefinable\xP@removePT@\relax
\ifcase\xP@digits
\def\xP@removePT@#1.#2#3@{\ifnum#2<5
#1\else
\the\numexpr-\if-#1-\else-#1+\fi\@ne\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5@{\ifnum#4<5
#1#2\if#30\else
.#3\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3pt+\if#1--\fi.12pt\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5#6@{\ifnum#5<5
#1#2\if#40\if#30\else
.#3\fi
\else
.#3#4\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3#4pt+\if#1--\fi786sp\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5#6#7@{\ifnum#6<5
#1#2\if#50\if#40\if#30\else
.#3\fi
\else
.#3#4\fi
\else
.#3#4#5\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3#4#5pt+\if#1--\fi79sp\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5#6#7#8@{\ifnum#7<5
#1#2\if#60\if#50\if#40\if#30\else
.#3\fi
\else
.#3#4\fi
\else
.#3#4#5\fi
\else
.#3#4#5#6\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3#4#5#6pt+\if#1--\fi8sp\relax
\fi
}
\else
\let\xP@dim\xP@precdim
\fi
\AtBeginDocument{{\setbox0\hbox{$ $}}\@ifdefinable\xP@lw\relax
\@ifdefinable\xP@preclw\relax
\edef\xP@preclw{\the\fontdimen8\textfont3}\edef\xP@lw{\xP@dim\xP@preclw}\PackageInfo{xypdf}{Line width: \xP@preclw}}
\xP@hook{pdf}{line@}
\newcommand*\xP@line@{\setboxz@h{\xP@setsolidpat
\xP@stroke{0 0 m \xP@coor{\cosDirection\xydashl@}{\sinDirection\xydashl@}l}}\U@c\sinDirection\xydashl@
\D@c\z@
\ifdim\U@c<\z@
\multiply\U@c\m@ne
\xP@swapdim\U@c\D@c
\fi
\ht\z@\U@c
\dp\z@\D@c
\R@c\cosDirection\xydashl@
\L@c\z@
\ifdim\R@c<\z@
\multiply\R@c\m@ne
\xP@swapdim\L@c\R@c
\fi
\hskip\L@c\boxz@\hskip\R@c
\edef\tmp@{\egroup\U@c\the\U@c\D@c\the\D@c\L@c\the\L@c\R@c\the\R@c}\tmp@
\Edge@c={\rectangleEdge}\edef\Upness@{\ifdim\z@<\U@c1\else0\fi}\edef\Leftness@{\ifdim\z@<\L@c1\else0\fi}\def\Drop@@{\styledboxz@}\def\Connect@@{\solid@}}
\xP@hook{pdf}{solid@}
\newcommand*\xP@solid@{\straight@\xP@solidSpread}
\@ifdefinable\xP@solidSpread\relax
\def\xP@solidSpread#1\repeat@{{\@tempswatrue
\ifdim\X@p=\X@c
\ifdim\Y@p=\Y@c
\@tempswafalse
\fi
\fi
\if@tempswa
\xP@setsolidpat
\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\X@c\Y@c l}\fi
}}
\newcommand*\xP@pattern{}
\newcommand*\xP@setsolidpat{\def\xP@pattern{1 J 1 j []0 d}\global\let\xP@lastpattern\xP@solidmacro
}
\newcommand*\xP@stroke[1]{\xP@literal{\xP@lw w \xP@pattern\space#1 S}}
\xP@hook{pdf}{dash@}
\newcommand\xP@dash@{\line@\def\Connect@@{\straight@\xP@dashedSpread}}
\@ifdefinable\xP@dashedSpread\relax
\def\xP@dashedSpread#1\repeat@{{\xP@veclen
\ifdim\@tempdimb>\z@
\xP@setdashpat
\xP@savec
\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\X@c\Y@c l}\fi
}}
\newcommand*\xP@setdashpat{\xP@testcont\xP@dashmacro
\ifxP@splinecont
{\count@\numexpr2*((\@tempdimb-\xydashl@/3)/(2*\xydashl@))\relax
\global\dimen@i
\ifnum\count@>\z@
\dimexpr\@tempdimb/\count@\relax
\else
\z@
\fi
}\@tempdima\dimen@i
\edef\xP@pattern{1 J 1 j [\ifdim\@tempdima>\z@
\xP@precdim\@tempdima]\xP@precdim\@tempdima
\else
]0 \fi
d}\else
\@tempdima
\ifdim\@tempdimb>\xydashl@
\dimexpr\@tempdimb/(2*((\@tempdimb+\xydashl@)/(2*\xydashl@))-1)\relax
\else
\z@
\fi
\edef\xP@pattern{1 J 1 j [\ifdim\@tempdima>\z@\xP@precdim\@tempdima\fi
]0 d}\fi
\global\let\xP@lastpattern\xP@dashmacro
}
\newcommand*\xP@setcldashpat{{\count@\numexpr2*((\@tempdimb-\xydashl@/3)/(2*\xydashl@))\relax
\xdef\@gtempa{1 J 1 j [\ifnum\count@>\z@\xP@precdim{\@tempdimb/\count@}\fi]\ifnum\count@>\z@\xP@precdim{\@tempdimb*3/2/\count@}\else0 \fi d}}\edef\xP@pattern{\@gtempa}}
\xP@hook{pdf}{point@}
\newcommand*\xP@point@{\xP@zerodot\egroup\Invisible@false
\Hidden@false\def\Leftness@{.5}\def\U@pness@{.5}\ctipEdge@
\def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\xP@dottedSpread}}
\newcommand*\xP@zerodot{\hb@xt@\z@{\hss
\vbox to\z@{\vss\hrule\@width\xP@preclw\@height\xP@preclw\vss}\hss}}
\@ifdefinable\xP@dottedSpread\relax
\def\xP@dottedSpread#1\repeat@{{\xP@veclen
\ifdim\@tempdimb>\z@
\xP@setdottedpat
\xP@savec
\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\X@c\Y@c l}\fi
}}
\newcommand*\xP@setdottedpat{\xP@testcont\xP@dotmacro
\ifxP@splinecont
\@tempdima\dimexpr\@tempdimb/(\@tempdimb/131072+1)-\xP@preclw\relax
\edef\xP@pattern{0 J [\ifdim\@tempdima>\z@
\xP@precdim\xP@preclw\xP@precdim\@tempdima
\fi
]\xP@precdim{\xP@preclw+1sp}d}\else
\advance\@tempdimb-\xP@preclw
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\@tempdima\dimexpr\@tempdimb/(\@tempdimb/131072+1)-\xP@preclw\relax
\edef\xP@pattern{0 J [\ifdim\@tempdima>\z@
\xP@precdim\xP@preclw\xP@precdim\@tempdima
\fi
]0 d}\fi
\global\let\xP@lastpattern\xP@dotmacro
}
\newcommand*\xP@setcldottedpat{\@tempdima\dimexpr\@tempdimb/(\@tempdimb/131072+1)-\xP@preclw\relax
\edef\xP@pattern{0 J [\ifdim\@tempdima>\z@
\xP@precdim\xP@preclw\xP@precdim\@tempdima
\fi
]\xP@precdim{\dimexpr\xP@preclw+\@tempdima/2\relax}d}}
\newcommand*\xP@abs[1]{\ifdim#1<\z@\multiply#1\m@ne\fi}
\newcommand*\xP@ifabsless[2]{\ifpdfabsdim#1<#2}
\ifx\ifpdfabsdim\@undefined
\renewcommand*\xP@ifabsless[2]{\ifdim\ifdim#1<\z@-\fi#1<\ifdim#2<\z@-\fi#2}
\@gobble\fi
\fi
\newcommand*\xP@swapdim[2]{\@tempdima#1#1#2#2\@tempdima}
\newcommand*\xP@swapnum[2]{\@tempcnta#1#1#2#2\@tempcnta}
\newcommand*\xP@min[2]{\ifdim#1<#2#1\else#2\fi}
\newcommand*\xP@max[2]{\ifdim#1>#2#1\else#2\fi}
\newcommand*\xP@Max[2]{#1\ifdim#2<\z@\xP@max#1{-#2}\else\xP@max#1#2\fi}
\newcommand*\xP@sqrt{\loop
\@tempdimb\dimexpr(\@tempdimc+(\@tempdima*\p@/\@tempdimc))/2\relax
\unless\ifdim\@tempdimc=\@tempdimb
\@tempdimc\@tempdimb\relax
\repeat
}
\newcommand*\xP@veclen{{\xP@veclen@
\global\dimen@i\@tempdimb
}\@tempdimb\dimen@i
}
\newcommand*\xP@veclen@{\xP@abs\d@Y
\ifdim\d@X=\z@
\@tempdimb\d@Y
\else
\xP@abs\d@X
\ifdim\d@Y=\z@
\@tempdimb\d@X
\else
\@tempswatrue
\ifdim\d@X>5931641sp\relax\@tempswafalse\fi
\ifdim\d@Y>5931641sp\relax\@tempswafalse\fi
\if@tempswa
\count@\@ne
\loop
\@tempdima\dimexpr\d@X*\d@X/\p@+\d@Y*\d@Y/\p@\relax
\ifdim\@tempdima<4096pt
\@tempcnta\ifdim\@tempdima<1024pt\ifdim\@tempdima<256pt8\else4\fi\else\tw@\fi
\multiply\d@X\@tempcnta
\multiply\d@Y\@tempcnta
\multiply\count@\@tempcnta
\repeat
\@tempdimc\dimexpr(\d@X+\d@Y)*3/4\relax
\xP@sqrt
\@tempdimb\dimexpr\@tempdimb/\count@\relax
\else
\ifdim\d@X>83042982sp\relax\@tempswatrue\fi
\ifdim\d@Y>83042982sp\relax\@tempswatrue\fi
\if@tempswa
\@tempdima\dimexpr\d@X/182*\d@X/11927552+\d@Y/182*\d@Y/11927552\relax
\@tempdimc\dimexpr(\d@X+\d@Y)*3/728\relax
\xP@sqrt
\multiply\@tempdimb182\relax
\else
\@tempdima\dimexpr\d@X*\d@X/12845056+\d@Y*\d@Y/12845056\relax
\@tempdimc\dimexpr(\d@X+\d@Y)*3/56\relax
\xP@sqrt
\multiply\@tempdimb14\relax
\fi
\fi
\fi
\fi
}
\xP@hook{pdf}{squiggledSpread@}
\@ifdefinable\xP@squiggledSpread@\relax
\def\xP@squiggledSpread@#1\repeat@{{\xP@veclen
\ifdim\@tempdimb>\z@
\edef\@tempa{\xP@coor\X@p\Y@p m }\toks@\expandafter{\@tempa}\@tempcnta\numexpr\@tempdimb/\xybsqll@\relax
\ifnum\@tempcnta<\tw@\@tempcnta\tw@\fi
\@tempdima\dimexpr\d@X/\@tempcnta\relax
\@tempdimc\dimexpr\d@Y/\@tempcnta\relax
\xP@testcont\xP@oddsquigglemacro
\ifxP@splinecont
\def\xP@squigsign{-}\else
\let\xP@squigsign\@empty
\fi
\count@\z@
\loop
\xP@append\toks@{\xP@coor{\X@p+\d@X*\count@/\@tempcnta+(\@tempdima
-\xP@squigsign\ifodd\count@-\fi\@tempdimc)*147546029/534618434}{\Y@p+\d@Y*\count@/\@tempcnta+(\@tempdimc
+\xP@squigsign\ifodd\count@-\fi\@tempdima)*147546029/534618434}}\advance\count@\@ne
\xP@append\toks@{\xP@coor{\X@p+\d@X*\count@/\@tempcnta-(\@tempdima
-\xP@squigsign\ifodd\count@-\fi\@tempdimc)*147546029/534618434}{\Y@p+\d@Y*\count@/\@tempcnta-(\@tempdimc
+\xP@squigsign\ifodd\count@-\fi\@tempdima)*147546029/534618434}\xP@coor{\X@p+\d@X*\count@/\@tempcnta}{\Y@p+\d@Y*\count@/\@tempcnta}c }\ifnum\count@<\@tempcnta
\repeat
\xP@setsolidpat
\global\expandafter\let\expandafter\xP@lastpattern
\ifodd\numexpr\count@\if\xP@squigsign-+1\fi\relax
\xP@oddsquigglemacro
\else
\xP@evensquigglemacro
\fi
\xP@savec
\xP@stroke{\the\toks@}\fi
}}
\newcommand*\xP@squigsign{}
\newcommand*\xP@append[2]{{\edef\@tempa{#1{\the#1#2}}\expandafter}\@tempa
}
\xP@hook{pdf}{circhar@@}
\newcommand*\xP@circhar@@[1]{\expandafter\xP@circhar@@@\ifcase#1 000{-173517671/654249180}{65307479/619869377}{-34221476/65864945}{225058681/768398401}{-543339720/768398401}\or
0{-543339720/768398401}{181455824/967576667}{-554561898/619869377}{826676217/1870772527}{-1}{543339720/768398401}{-1}\or
0{-1}{173517671/654249180}{-1}{34221476/65864945}{-554561898/619869377}{543339720/768398401}{-543339720/768398401}\or
0{-543339720/768398401}{181455824/967576667}{-34221476/65864945}{225058681/768398401}{-173517671/654249180}{225058681/768398401}0\or
0{543339720/768398401}{181455824/967576667}{34221476/65864945}{225058681/768398401}{173517671/654249180}{225058681/768398401}0\or
01{173517671/654249180}1{34221476/65864945}{554561898/619869377}{543339720/768398401}{543339720/768398401}\or
0{543339720/768398401}{181455824/967576667}{554561898/619869377}{826676217/1870772527}1{543339720/768398401}1\or
000{173517671/654249180}{65307479/619869377}{34221476/65864945}{225058681/768398401}{543339720/768398401}\fi}
\newcommand\xP@circhar@@@[8]{\xP@setsolidpat
\xP@stroke{\xP@coor{\R@*#1}{\R@*#2}m
\xP@coor{\R@*#3}{\R@*#4}\xP@coor{\R@*#5}{\R@*#6}\xP@coor{\R@*#7}{\R@*#8}c}\vrule width\z@ height\R@ depth\R@
\kern\dimexpr\R@*#7\relax
}
\xP@hook{pdf}{cirrestrict@@}
\newcommand*\xP@cirrestrict@@{\count@\z@\relax}
\newcommand*\xP@trigfromdir[1]{{\Direction#1\relax
\count@-\Direction
\advance\count@4096
\divide\count@2048
\ifcase\count@
\d@X\K@\p@
\d@Y\numexpr\Direction-3*\K@\relax\p@
\or
\d@X\numexpr\Direction-\K@\relax\p@
\d@Y-\K@\p@
\or
\d@X-\K@\p@
\d@Y\numexpr-\Direction-\K@\relax\p@
\or
\d@X\numexpr-\Direction-3*\K@\relax\p@
\d@Y\K@\p@
\else
\PackageError{xypdf}{Unexpected case in direction calculation}{Feel free to contact the author of the xypdf package with a minimal example.}\fi
\xP@veclen
\xdef\@gtempa{\def\noexpand\cosDirection{\xP@EARPT\dimexpr\d@X*\p@/\@tempdimb\relax}\def\noexpand\sinDirection{\xP@EARPT\dimexpr\d@Y*\p@/\@tempdimb\relax}}}\@gtempa
}
\outer\def\@tempa{\alloc@1\dimen\dimendef\insc@unt}
\let\xP@newdimen\newdimen
\ifx\newdimen\@tempa
\def\xP@newdimen{\alloc@1\dimen\dimendef\insc@unt}
\fi
\outer\def\@tempa#1{\count@=\escapechar\escapechar=-1
\expandafter\expandafter\expandafter
\def\@if#1{true}{\let#1=\iftrue}\expandafter\expandafter\expandafter
\def\@if#1{false}{\let#1=\iffalse}\@if#1{false}\escapechar=\count@}
\let\@tempa\relax
\newcommand*\xP@lastX{}
\newcommand*\xP@lastY{}
\newcommand*\xP@lastpattern{}
\newcommand*\xP@solidmacro{solid}
\newcommand*\xP@dotmacro{dot}
\newcommand*\xP@dashmacro{dash}
\newcommand*\xP@evensquigglemacro{evensquiggle}
\newcommand*\xP@oddsquigglemacro{oddsquiggle}
\newcommand*\xP@brokensquigglemacro{brokensquiggle}
\renewcommand*\xyinside@{\global\let\xP@lastpattern\@empty
\saveXyStyle@ \aftergroup\xycheck@end
\setboxz@h\bgroup
\plainxy@
\X@c=\z@\Y@c=\z@\czeroEdge@
\X@p=\z@\Y@p=\z@\U@p=\z@\D@p=\z@\L@p=\z@\R@p=\z@\Edge@p={\zeroEdge}\X@min=\hsize\X@max=-\hsize\Y@min=\hsize\Y@max=-\hsize
\mathsurround=\z@
\expandafter\POS\everyxy@@
}
\newcommand*\xP@savec{\xdef\xP@lastX{\the\X@c}\xdef\xP@lastY{\the\Y@c}}
\@ifdefinable\ifxP@splinecont\relax
\@ifdefinable\xP@splineconttrue\relax
\@ifdefinable\xP@splinecontfalse\relax
\newif\ifxP@splinecont
\newcommand*\xP@testcont[1]{\xP@splinecontfalse
\ifxP@cont
\ifx\xP@lastpattern#1\ifdim\xP@lastX=\X@p
\ifdim\xP@lastY=\Y@p
\xP@splineconttrue
\fi
\fi
\fi
\fi
}
\@ifdefinable\ifxP@cont\relax
\@ifdefinable\xP@conttrue\relax
\@ifdefinable\xP@contfalse\relax
\newif\ifxP@cont
\newcommand*\xypdfcontpatternon{\xP@conttrue}
\newcommand*\xypdfcontpatternoff{\xP@contfalse}
\xP@conttrue
\let\@tempa\@undefined
\let\nextii@\@undefined
\DN@{\xywithoption{color}{\message{Xy-pic pdf driver: `color' extension support}\@ifundefined{xypdf-co@loaded}{\input xypdf-co\relax}{\message{not reloaded}}}\xywithoption{curve}{\message{Xy-pic pdf driver: `curve' extension support}\@ifundefined{xypdf-cu@loaded}{\input xypdf-cu\relax}{\message{not reloaded}}}\xywithoption{frame}{\message{Xy-pic pdf driver: `frame' extension support}\@ifundefined{xypdf-fr@loaded}{\input xypdf-fr\relax}{\message{not reloaded}}}\xywithoption{line}{\message{Xy-pic pdf driver: `line' extension support}\@ifundefined{xypdf-li@loaded}{\input xypdf-li\relax}{\message{not reloaded}}}\xywithoption{rotate}{\message{Xy-pic pdf driver: `rotate' extension support}\@ifundefined{xypdf-ro@loaded}{\input xypdf-ro\relax}{\message{not reloaded}}}}
\next@
\xyendinput
%%
%% End of file `xypdf.tex'.

